FedNest: Federated Bilevel, Minimax, and Compositional Optimization

Standard federated optimization methods successfully apply to stochastic problems with single-level structure. However, many contemporary ML problems -- including adversarial robustness, hyperparameter tuning, and actor-critic -- fall under nested bilevel programming that subsumes minimax and compositional optimization. In this work, we propose \fedblo: A federated alternating stochastic gradient method to address general nested problems. We establish provable convergence rates for \fedblo in the presence of heterogeneous data and introduce variations for bilevel, minimax, and compositional optimization. \fedblo introduces multiple innovations including federated hypergradient computation and variance reduction to address inner-level heterogeneity. We complement our theory with experiments on hyperparameter \& hyper-representation learning and minimax optimization that demonstrate the benefits of our method in practice. Code is available at https://github.com/ucr-optml/FedNest.

==> FedNest_ _/icml/notation_icml.tex <==
% Recommended, but optional, packages for figures and better typesetting:
\usepackage{microtype,bm}
\usepackage{graphicx}
%\usepackage{subfigure}
\usepackage{booktabs} % for professional tables

\usepackage{hyperref}

% For theorems and such
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{amsthm}
\usepackage{caption}

% if you use cleveref..
\usepackage[capitalize,noabbrev]{cleveref}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% THEOREMS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\theoremstyle{plain}

% Todonotes is useful during development; simply uncomment the next line
%    and comment out the line below the next line to turn off comments
%\usepackage[disable,textsize=tiny]{todonotes}
\usepackage[textsize=tiny]{todonotes}



%%%%%%%%%%%%%%%%%%%%
%%%% GENERAL PACKAGES %%%%
%%%%%%%%%%%%%%%%%%%%
%\usepackage[margin=1in]{geometry}
%\renewcommand{\baselinestretch}{1.5}	% Line Stretch
\usepackage{color}
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{natbib}
%\usepackage[colorlinks,citecolor=blue,linkcolor=blue,urlcolor=blue]{hyperref}
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{booktabs}
%\usepackage[table,x11names,dvipsnames,table]{xcolor}
\usepackage[rightcaption]{sidecap}
\sidecaptionvpos{figure}{c}
\usepackage{bbm}
\usepackage{latexsym, epsfig, amssymb, amsmath, amsthm, mathrsfs, booktabs,mathtools}
\usepackage{enumerate}
\usepackage{multirow}
\usepackage{multicol}
\usepackage{array,booktabs}
\usepackage{enumitem}
\usepackage{epstopdf}
\usepackage{subcaption}
\usepackage{wrapfig}
\usepackage{adjustbox}
\usepackage{multirow}
\usepackage{multicol}
\usepackage{array,booktabs}
%\usepackage{algorithm}
\usepackage{algpseudocode} 
\usepackage{enumitem}
\usepackage{epstopdf}
\usepackage{xspace}
\usepackage{comment}
\usepackage{multirow}
\usepackage{makecell}

%%%%%%%% To add checkbox support%%%%%
\usepackage{enumitem,amssymb}
\usepackage{pifont}
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%
\newcommand{\checkbox}{\rlap{$\square$}{\raisebox{2pt}{\large\hspace{1pt}\cmark}}%
\hspace{2.5pt}}
%%%%%%%%%%% end checkbox %%%%%%%%%

%\setlength{\footskip}{3.30003pt}
%%%
%%
\newenvironment{myitemize}{\begin{list}{$\bullet$}
		{\setlength{\topsep}{1mm}
			\setlength{\itemsep}{0.25mm}
			\setlength{\parsep}{0.25mm}
			\setlength{\itemindent}{0mm}
			\setlength{\partopsep}{0mm}
			\setlength{\labelwidth}{15mm}
			\setlength{\leftmargin}{4mm}}}{\end{list}}
%\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\renewcommand{\algorithmicrequire}{ \textbf{Input:}}
\renewcommand{\algorithmicensure}{ \textbf{Output:}}
\newcommand\inner[2]{\langle #1, #2 \rangle}
%%%%%
%%%% notation %%%%%%%%%%%%%%%%
\newcommand{\mc}{\mathcal}
\newcommand{\E}{\mb{E}}
\newcommand{\m}[1]{{\bm{#1}}}
\newcommand{\wh}[1]{{\widehat{#1}}}
\newcommand{\un}[1]{{\underline{#1}}}
\newcommand{\ti}[1]{{\tilde{#1}}}
\newcommand{\fedurl}{github.com/mc-nya/FedNest}
\renewcommand{\mc}[1]{\ensuremath{\mathcal{#1}}} 
\newcommand{\g}[1]{\mbox{\boldmath $#1$}}
\newcommand{\mb}[1]{{\mathbb{#1}}}
\newcommand{\V}[1]{\ensuremath{\boldsymbol{#1}}\xspace}
\newcommand{\M}[1]{\ensuremath{\boldsymbol{#1}}\xspace}
%% Math Functions
\newcommand{\F}[1]{\ensuremath{\mathrm{#1}}\xspace}
\newcommand{\sgn}{\F{sgn}}
\newcommand{\tr}{\F{trace}}
\newcommand{\minmax}{minimax}
\newcommand{\Minmax}{Minimax}
%\newcommand{\text{diag}}{\F{diag}}
\newcommand{\dett}{\F{det}}
%\DeclareMathOperator*{\argmax}{\arg\!\max}
%\DeclareMathOperator*{\argmin}{\arg\!\min}
\DeclarePairedDelimiterX{\norm}[1]{\lVert}{\rVert}{#1}
\newcommand*{\Scale}[2][4]{\scalebox{#1}{$#2$}}
%% Transpose
%%%%% operator%%%%%%%%%%%% 
\DeclareMathOperator*{\minimize}{minimize}
%\DeclareMathOperator{\text{diag}}{diag}
\DeclareMathOperator{\trace}{trace}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\eig}{eig}
\DeclareMathOperator{\logt}{logdet}
\DeclareMathOperator{\Var}{Var}
%%%%%%%%%%% theorem %%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\Lmax}{\ensuremath{L^\ast}}
\newcommand{\Lsum}{\overline{L}}
\newcommand{\ellmin}{\ensuremath{\ell_\ast}}
\newcommand{\proxjplain}{ {\mathtt{prox\_update}}_j}
\newcommand{\proxj}[1]{\ensuremath{\proxjplain(#1)}}
\newcommand{\zfp}{z^\star}
\DeclareMathOperator{\refl}{\bf refl}
\newcommand{\aprox}{\widetilde{\prox}}
\newcommand{\aproxj}[2]{\mathtt{prox\_update}_{#1}(#2)}
\newcommand{\arefl}{\widetilde{\refl}}
\newcommand{\eqset}{E}
\newcommand{\Orthog}{\ensuremath{\mathrm{O}}}
\newcommand{\zstar}{z^\star}
\definecolor{darkred}{RGB}{150,0,0}
\definecolor{darkgreen}{RGB}{0,150,0}
\definecolor{darkblue}{RGB}{0,0,200}
\hypersetup{colorlinks=true, linkcolor=darkred, citecolor=darkgreen, urlcolor=darkblue}
\newcommand{\som}[1]{\marginpar{\color{darkred}\tiny\ttfamily SO: #1}}
\newcommand{\so}[1]{\textcolor{darkred}{#1}}
\newcommand{\SO}[1]{\textcolor{darkred}{SO: #1}}
\let\phi\varphi
\newcommand{\Unif}{\ensuremath{\mathsf{Unif}}}
\newcommand{\numepoch}{\numepochs}
\newcommand{\defn}{\ensuremath{\coloneq}}
%%%%
\newcommand{\eps}{\varepsilon}
\newtheorem{theorem}{Theorem}[section] %[section]
\newtheorem{lemma}{Lemma}[section] %[section]
\newtheorem{corollary}{Corollary}[section] %[section]
\newtheorem{proposition}{Proposition}[section] %[section]
\newtheorem{definition}{Definition}[section] %[section]
\newtheorem{remark}{Remark}[section]%[section]
\newtheorem{example}{Example} %[section]
\newtheorem{assumption}{Assumption}
\renewcommand*{\theassumption}{\Alph{assumption}}
\newcommand{\lall}[1]{{\order{\lip_{\lan #1}}}}
\newcommand{\order}[1]{{\cal{O}}(#1)}
%--------------------------------------------------------------
% Full names of federated algorithms
\newcommand{\fedblo}{\textsc{FedNest}\xspace}
\newcommand{\lfedblo}{\textsc{LFedNest}\xspace}
\newcommand{\Blo}{Bilevel}
\newcommand{\blo}{bilevel}
\newcommand{\nn}{\nonumber}
\newcommand{\fed}{\textsc{Fed}\xspace}
\newcommand{\fadagrad}{\textsc{FedAdagrad}\xspace}
\newcommand{\fedavg}{\textsc{FedAvg}\xspace}
\newcommand{\fedavgm}{\textsc{FedAvgM}\xspace}
\newcommand{\fedopt}{\textsc{FedOpt}\xspace}
\newcommand{\fedesj}{\textsc{FedEsj}\xspace}
\newcommand{\fedsvrg}{\textsc{FedSVRG}\xspace}
\newcommand{\scaffold}{\textsc{SCAFFOLD}\xspace}
\newcommand{\adaalter}{\textsc{AdaAlter}\xspace}
\newcommand{\lookahead}{\textsc{Lookahead}\xspace}
\newcommand{\fedgrad}{\textsc{ApproxInverseHVP}\xspace}
\newcommand{\fedminmax}{\textsc{FedMinMax}\xspace}
\newcommand{\fedcomp}{\textsc{FedComp}\xspace}
\newcommand{\fedinn}{\textsc{FedInn}\xspace}
\newcommand{\fedout}{\textsc{FedOut}\xspace}
\newcommand{\lfedinn}{\textsc{LFedInn}\xspace}
\newcommand{\lfedout}{\textsc{LFedOut}\xspace}
\newcommand{\fednest}{\textsc{FedNest}\xspace}
\newcommand{\fedhess}{\textsc{FedIHGP}\xspace}
\newcommand{\joint}{\textsc{{LFedNest}}-\text{NonAlt}\xspace}
\newcommand{\vct}[1]{\bm{#1}}
\newcommand{\mtx}[1]{\bm{#1}}
\newcommand{\x}{\vct{x}}
\newcommand{\y}{\vct{y}}
\newcommand{\red}{\textcolor{darkred}}

\newcommand{\funcin}{\mathbb{G}}%{\textsc{Func}}
\newcommand{\funco}{\mathbb{F}}%{\textsc{Func}}

%% Notation for comment %%
\newcommand{\mli}[1]{{\color{blue}#1}}

==> FedNest_ _/notation.tex <==
\usepackage[margin=1in]{geometry}
\renewcommand{\baselinestretch}{1.5}	% Line Stretch
\usepackage{color}
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{natbib}
\usepackage{caption}
\usepackage{longtable}
\usepackage{boldline}
% \usepackage[toc,page,header]{appendix}
% \usepackage{minitoc}
% Make the "Part I" text invisible
\renewcommand \thepart{}
\renewcommand \partname{}
\usepackage[colorlinks,citecolor=blue,linkcolor=blue,urlcolor=blue]{hyperref}
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{booktabs}
\usepackage[table,x11names,dvipsnames,table]{xcolor}
\usepackage{graphicx}
\usepackage{wrapfig}
\usepackage[rightcaption]{sidecap}
\sidecaptionvpos{figure}{c}
\usepackage{bbm}
\usepackage{latexsym, epsfig, amssymb, amsmath, amsthm, graphicx, mathrsfs, booktabs,mathtools}
\usepackage{enumerate}
\usepackage{multirow}
\usepackage{multicol}
\usepackage{array,booktabs}
\usepackage{enumitem}
\usepackage{epstopdf}
\usepackage{subcaption}
\usepackage{wrapfig}
\usepackage{adjustbox}
\usepackage{multirow}
\usepackage{multicol}
\usepackage{array,booktabs}
\usepackage{algorithm}
\usepackage{algpseudocode} 
\usepackage{enumitem}
\usepackage{epstopdf}
\usepackage{xspace}
\usepackage{comment}
\usepackage{multirow}
\usepackage{makecell}
\newcommand{\vct}[1]{\bm{#1}}
\newcommand{\mtx}[1]{\bm{#1}}
\newcommand{\x}{\vct{x}}
\newcommand{\y}{\vct{y}}


%%%
%%
%\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\renewcommand{\algorithmicrequire}{ \textbf{Input:}}
\renewcommand{\algorithmicensure}{ \textbf{Output:}}
\newcommand\inner[2]{\langle #1, #2 \rangle}
%%%%%
%%%% notation %%%%%%%%%%%%%%%%
\newcommand{\mc}{\mathcal}
\newcommand{\m}[1]{{\bf{#1}}}
\newcommand{\wh}[1]{{\widehat{#1}}}
\newcommand{\un}[1]{{\underline{#1}}}
\newcommand{\ti}[1]{{\tilde{#1}}}
\renewcommand{\mc}[1]{\ensuremath{\mathcal{#1}}} 
\newcommand{\g}[1]{\mbox{\boldmath $#1$}}
\newcommand{\mb}[1]{{\mathbb{#1}}}
\newcommand{\V}[1]{\ensuremath{\boldsymbol{#1}}\xspace}
\newcommand{\M}[1]{\ensuremath{\boldsymbol{#1}}\xspace}
%% Math Functions
\newcommand{\F}[1]{\ensuremath{\mathrm{#1}}\xspace}
\newcommand{\sgn}{\F{sgn}}
\newcommand{\tr}{\F{trace}}
%\newcommand{\text{diag}}{\F{diag}}
\newcommand{\dett}{\F{det}}
%\DeclareMathOperator*{\argmax}{\arg\!\max}
%\DeclareMathOperator*{\argmin}{\arg\!\min}
\DeclarePairedDelimiterX{\norm}[1]{\lVert}{\rVert}{#1}
\newcommand*{\Scale}[2][4]{\scalebox{#1}{$#2$}}
%% Transpose
%%%%% operator%%%%%%%%%%%% 
\DeclareMathOperator*{\minimize}{minimize}
%\DeclareMathOperator{\text{diag}}{diag}
\DeclareMathOperator{\trace}{trace}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\eig}{eig}
\DeclareMathOperator{\logt}{logdet}
\DeclareMathOperator{\Var}{Var}
%%%%%%%%%%% theorem %%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\Lmax}{\ensuremath{L^\ast}}
\newcommand{\Lsum}{\overline{L}}
\newcommand{\ellmin}{\ensuremath{\ell_\ast}}
\newcommand{\proxjplain}{ {\mathtt{prox\_update}}_j}
\newcommand{\proxj}[1]{\ensuremath{\proxjplain(#1)}}
\newcommand{\zfp}{z^\star}
\DeclareMathOperator{\refl}{\bf refl}
\newcommand{\aprox}{\widetilde{\prox}}
\newcommand{\aproxj}[2]{\mathtt{prox\_update}_{#1}(#2)}
\newcommand{\arefl}{\widetilde{\refl}}
\newcommand{\eqset}{E}
\newcommand{\Orthog}{\ensuremath{\mathrm{O}}}
\newcommand{\zstar}{z^\star}
\definecolor{darkred}{RGB}{150,0,0}
\definecolor{darkgreen}{RGB}{0,150,0}
\definecolor{darkblue}{RGB}{0,0,200}
\hypersetup{colorlinks=true, linkcolor=darkred, citecolor=darkgreen, urlcolor=darkblue}
\newcommand{\som}[1]{\marginpar{\color{darkred}\tiny\ttfamily SO: #1}}
\newcommand{\so}[1]{\textcolor{darkred}{#1}}
\newcommand{\SO}[1]{\textcolor{darkred}{SO: #1}}
\let\phi\varphi
\newcommand{\Unif}{\ensuremath{\mathsf{Unif}}}
\newcommand{\numepoch}{\numepochs}
\newcommand{\defn}{\ensuremath{\coloneq}}
%%%%
\newtheorem{theorem}{Theorem}[section] %[section]
\newtheorem{lemma}{Lemma}[section] %[section]
\newtheorem{corollary}{Corollary}[section] %[section]
\newtheorem{proposition}{Proposition}[section] %[section]
\newtheorem{definition}{Definition}[section] %[section]
\newtheorem{remark}{Remark}[section]%[section]
\newtheorem{example}{Example}[section] %[section]
\newtheorem{assumption}{Assumption}
\renewcommand*{\theassumption}{\Alph{assumption}}
%--------------------------------------------------------------
\newenvironment{myitemize}{\begin{list}{$\bullet$}
		{\setlength{\topsep}{1mm}
			\setlength{\itemsep}{0.25mm}
			\setlength{\parsep}{0.25mm}
			\setlength{\itemindent}{0mm}
			\setlength{\partopsep}{0mm}
			\setlength{\labelwidth}{15mm}
			\setlength{\leftmargin}{4mm}}}{\end{list}}

% Full names of federated algorithms
\newcommand{\fedblo}{\textsc{FedNest}\xspace}
\newcommand{\Blo}{Bilevel}
\newcommand{\blo}{bilevel}
\newcommand{\nn}{\nonumber}
\newcommand{\fed}{\textsc{Fed}\xspace}
\newcommand{\fadagrad}{\textsc{FedAdagrad}\xspace}
\newcommand{\fedavg}{\textsc{FedAvg}\xspace}
\newcommand{\fedavgm}{\textsc{FedAvgM}\xspace}
\newcommand{\fedopt}{\textsc{FedOpt}\xspace}
\newcommand{\fedesj}{\textsc{FedEsj}\xspace}
\newcommand{\fedsvrg}{\textsc{FedSVRG}\xspace}
\newcommand{\scaffold}{\textsc{SCAFFOLD}\xspace}
\newcommand{\adaalter}{\textsc{AdaAlter}\xspace}
\newcommand{\lookahead}{\textsc{Lookahead}\xspace}
\newcommand{\fedgrad}{\textsc{ApproxInverseHVP}\xspace}
\newcommand{\fedminmax}{\textsc{FedMinMax}\xspace}
\newcommand{\fedcomp}{\textsc{FedComp}\xspace}
\newcommand{\fedinn}{\textsc{FedInn}\xspace}
\newcommand{\fedout}{\textsc{FedOut}\xspace}
\newcommand{\fednest}{\textsc{FedNest}\xspace}
\newcommand{\fedhess}{\textsc{FedIHGP}\xspace}

==> FedNest_ _/sec/abstract.tex <==
\begin{abstract}
%Federated learning is a distributed machine learning paradigm in which a large number of clients coordinate with a central server to learn a model without sharing their own training data. 
Standard federated optimization methods successfully apply to stochastic problems with \textit{single-level} structure. However, many contemporary ML problems -- including adversarial robustness, hyperparameter tuning, actor-critic -- fall under nested bilevel programming that subsumes minimax and compositional optimization. In this work, we propose \fedblo: A federated alternating stochastic gradient method to address general nested problems. We establish provable convergence rates for \fedblo in the presence of heterogeneous data and introduce variations for bilevel, minimax, and compositional optimization. \fedblo introduces multiple innovations including federated hypergradient computation and variance reduction to address inner-level heterogeneity. We complement our theory with experiments on hyperparameter \& hyper-representation learning and minimax optimization that demonstrate the benefits of our method in practice.  Code is available at \url{https://github.com/ucr-optml/FedNest}.
%\url{\fedurl}.}
% and adversarial learning
\end{abstract}

==> FedNest_ _/sec/actor_critic.tex <==
% \section{Application to Federated Actor-Critic}

% We will follow the exposition of the prior convergence results on actor-critic methods \cite{chen2021closing,hong2020two}.





==> FedNest_ _/sec/algos.tex <==
\subsection{Proposed Algorithm: \fedblo}

In this section, we develop \fedblo, which is formally presented in Algorithm \ref{alg:fedblo}. The algorithm operates in two nested loops. The outer loop operates in rounds $k\in\{1,\ldots,K\}$. Within each round, an inner loop operating for $T$ iterations is executed. Given estimates $\m{x}^k$ and  $\m{y}^k$, each iteration $t\in\{1,\ldots,T\}$ of the inner loop produces a new \emph{global} model $\m{y}^{k,t+1}$ of the inner optimization variable $\m{y}^*(\m{x}^k)$ as the output of an optimizer \fedinn. The final estimate $\m{y}^{k+1}=\m{y}^{k,T}$ of the inner variable is then used by an optimizer \fedout to update the outer \emph{global} model $\m{x}^{k+1}$.


The subroutines \fedinn and \fedout are gradient-based optimizers.
%that perform \emph{local} updates.
Each subroutine involves a certain number of \emph{local} training steps indexed by $\nu\in\{0,\ldots,\tau_i-1\}$ that are performed at the $i^{\text{th}}$ client. The local steps of \fedinn iterate over \emph{local} models $\m{y}_{i,\nu }$ of the inner variable. Accordingly, \fedout iterates over \emph{local} models $\m{x}_{i,\nu }$ of the global variable. A critical component of \fedout is a communication-efficient federated hypergradient estimation routine, which we call {\fedhess}.
%
The implementation of \fedinn, \fedout and \fedhess is critical to circumvent the algorithmic challenges of federated bilevel optimization. In the remaining of this section, we detail the challenges and motivate our proposed implementations. Later, in Section \ref{sec:theory}, we provide a formal convergence analysis of \fednest. 
%
\subsection{Key Challenge: Federated Hypergradient Estimation}\label{sec:fedhess}

\fedout is a gradient-based optimizer for the outer minimization in \eqref{fedblo:prob}; thus each iteration involves computing $\nabla f(\x)=(1/m)\sum_{i=1}^{m}\nabla f_i(\x,\y^*(\x))$. Unlike single-level FL, the fact that the outer objective $f$ depends explicitly on the inner minimizer $\y^*(\x)$ introduces a new challenge. 
%
%
A good starting point to understand the challenge is the following evaluation of $\nabla f(\x)$ in terms of partial derivatives. The result is well-known from properties of implicit functions.
%
\begin{lemma}\label{lem:IFT}
Under Assumption~\ref{assu:f}, for all $i\in [m]$:
\begin{subequations}\label{main_grad}
\begin{align*}
\nabla f_i(\m{x}, \m{y}^*(\m{x}))&= \nabla^{\texttt{D}}f_i\left(\m{x},\m{y}^*(\m{x})\right)+\nabla^{\texttt{I}}f_i\left(\m{x},\m{y}^*(\m{x})\right),
\end{align*}
%\ct{$-$ sign above?}
where the \emph{direct} and \emph{indirect} gradient components are:
\begin{align}\label{main_grad:decom}
&  \nabla^{\texttt{D}} f_i(\m{x},\m{y}^*(\m{x})):= \nabla_{\m{x}}f_i\left(\m{x},\m{y}^*(\m{x})\right),\\
\nonumber
&\nabla^{\texttt{I}} f_i(\m{x},\m{y}^*(\m{x})):=- \nabla^2_{\m{x}\m{y}} g(\m{x},\m{y}^*(\m{x}))\\
&\quad \qquad\cdot \left[\nabla^2_{\m{y}}g(\m{x},\m{y}^*(\m{x}))\right]^{-1} \nabla_\m{y} f_i \left(\m{x},\m{y}^*(\m{x})\right).\label{main_grad:decom2}
\end{align}
\end{subequations}
\end{lemma}
We now use the above formula  
%on obtaining an unbiased stochastic estimate of $ \nabla f_i(\m{x}, \m{y}^*(\m{x}))$ 
to describe the two core challenges of bilevel FL optimization. 
%

First, evaluation of any of the terms in \eqref{main_grad} requires access to the minimizer $\m{y}^*(\m{x})$ of the inner problem. On the other hand, one may at best hope for a good \emph{approximation} to $\m{y}^*(\m{x})$ produced by the inner optimization subroutine. Of course, this challenge is inherent in any bilevel optimization setting, but is exacerbated in the FL setting because of \emph{client drift}. Specifically, when clients optimize their individual (possibly different) local inner objectives, the global estimate of the inner variable produced by SGD-type methods may drift far from (a good approximation to) $\m{y}^*(\m{x})$. We explain in Section \ref{sec:fedinn} how \fedinn solves that issue.
%

The second challenge comes from the stochastic nature of the problem. 
%and the distributed nature of local computations in a FL setting. 
Observe that the indirect component in \eqref{main_grad:decom2} is nonlinear in the Hessian $\nabla_{\m{y}}^2 g(\m{x}, \m{y}^*(\m{x}))$,   complicating an unbiased stochastic approximation of $\nabla f_i(\m{x}, \m{y}^*(\m{x}))$. As we expose here,  solutions to this complication developed in the non-federated bilevel optimization literature, are \emph{not} directly applicable in the FL setting. Indeed, existing stochastic bilevel algorithms, e.g.  \cite{ghadimi2018approximation}, define $\bar{\nabla}f(\m{x},\m{y}):= \bar{\nabla}^{\texttt{D}}f(\m{x},\m{y})+\bar{\nabla}^{\texttt{I}}f(\m{x},\m{y})$ as a surrogate of $\nabla f(\m{x},  \m{y}^*(\m{x}))$ by replacing $\m{y}^*(\m{x})$ in definition \eqref{main_grad} with an approximation $\m{y}$ and using the following stochastic approximations:
\begin{subequations}\label{eq.inverse-estimator}
\begin{align}\label{eq.inverse-estimator.a}
& \bar{\nabla}^{\texttt{D}}f(\m{x},\m{y})  \approx  \nabla_{\m{x}} f(\m{x}, \m{y};\dot{\xi}),
\\
\nonumber
& \bar{\nabla}^{\texttt{I}}f(\m{x},\m{y})  \approx  -\nabla^2_{\m{xy}}g(\m{x},\m{y};\zeta_{N'+1}) \\
& \Big[\frac{N}{\ell_{g,1}}\prod\limits_{n=1}^{N'}\big(\m{I}-\frac{1}{\ell_{g,1}} \nabla^2_{\m{y}} g(\m{x},\m{y};\zeta_n)\big)\Big] \nabla_\m{y} f(\m{x},\m{y};\dot{\xi}).
\label{eq.inverse-estimator.b}
\end{align}
\end{subequations}
Here, $N'$ is drawn from $\{0,  \ldots, N-1\}$ uniformly at random (UAR) and  $\{\dot{\xi}, \zeta_{1}, \ldots,\zeta_{N'+1}\}$ are i.i.d.~samples. 
\citet{ghadimi2018approximation,hong2020two} have shown that using \eqref{eq.inverse-estimator}, the inverse Hessian estimation bias exponentially decreases with the number of samples $N$. 

One might hope to directly leverage the above approach in a local computation fashion by replacing the global outer function $f$ with the individual function $f_i$. However, note from \eqref{main_grad:decom2} and \eqref{eq.inverse-estimator.b} that the proposed stochastic approximation of the indirect gradient involves in a nonlinear way the \emph{global} Hessian,  which is \emph{not} available at the client \footnote{We note that the approximation in \eqref{eq.inverse-estimator} is not the only construction, and bilevel optimization can accommodate other forms of gradient surrogates~\citep{ji2021bilevel}. Yet, all these approximations require access (in a nonlinear fashion) to the \emph{global} Hessian; thus, they suffer from the same challenge in FL setting.}. Communication efficiency is one of the core objectives of FL making the idea of communicating Hessians between clients and server prohibitive. \emph{Is it then possible, in a FL setting, to obtain an accurate stochastic estimate of the indirect gradient while retaining communication efficiency?} In Section \ref{sec:fedout}, we show how \fedout and its subroutine \fedhess, a matrix-vector products-based (thus, communication efficient) federated hypergradient estimator, answer this question affirmatively.
%However, in our case, problem is more daunting as the Hessian is distributed across users and classical Hessian approximations are not applicable.
% % One will notice from the above formula that obtaining an unbiased stochastic estimate of $ \nabla f_i(\m{x}, \m{y}^*(\m{x}))$ and applying SGD-type methods on $\m{x}$ face two main challenges: (i) the gradient $\nabla f_i(\m{x}, \m{y}^*(\m{x}))$ at $\m{x}$ depends on the minimizer of the inner problem $\m{y}^*(\m{x})$; (ii) even if $\m{y}^*(\m{x})$ is known, it is hard to apply the stochastic approximation to obtain an unbiased estimate of $\nabla f_i(\m{x}, \m{y}^*(\m{x}))$ since $\nabla f_i(\m{x}, \m{y}^*(\m{x}))$ is nonlinear in the Hessian $\nabla_{\m{y}}^2 g(\m{x}, \m{y}^*(\m{x}))$. 



% To address these issues, existing stochastic bilevel algorithms \citep{ghadimi2018approximation,hong2020two} define $\bar{\nabla}f(\m{x},\m{y})$ as a surrogate of $\nabla f(\m{x},  \m{y}^*(\m{x}))$ by replacing $\m{y}^*(\m{x})$ in definition \eqref{main_grad} with $\m{y}$ as follows
% \begin{align}\nonumber%\label{eq:bar:gradient}
% \bar{\nabla}f(\m{x},\m{y}) := & \bar{\m{h}}^{\texttt{dir}}(\m{x},\m{y})+\bar{\m{h}}^{\texttt{indir}}(\m{x},\m{y}).
% \end{align}
% %where 
% % \begin{align}\nonumber%\label{eq:bar:gradient}
% % \nabla_\m{x} f(\m{x},\m{y}) -  \\
% % &\nabla^2_{\m{x}\m{y}} g(\m{x},\m{y})[\nabla^2_{\m{y}}g(\m{x},\m{y})]^{-1} \nabla_\m{y} f(\m{x},\m{y}).\nonumber
% % \end{align} 
% Here,  $\bar{\m{h}}^{\texttt{dir}}(\m{x},\m{y})$ and $\bar{\m{h}}^{\texttt{indir}}(\m{x},\m{y})$ are surrogates of direct and indirect gradients, respectively. In non-federated homogeneous setting, they also stochastically estimate  $\bar{\m{h}}^{\texttt{dir}}(\m{x},\m{y})$ and $\bar{\m{h}}^{\texttt{indir}}(\m{x},\m{y})$ as follows
% \begin{subequations}
% \begin{align}\label{eq.inverse-estimator}
% &  \bar{\m{h}}^{\texttt{dir}}(\m{x},\m{y})  \approx \m{h}^{\texttt{dir}}(\m{x},\m{y})  := \nabla_{\m{x}} f(\m{x}, \m{y}, \xi)
% \\
%  \nonumber
% & \bar{\m{h}}^{\texttt{dir}}(\m{x},\m{y})  \approx  \m{h}^{\texttt{indir}}(\m{x},\m{y}) := -\nabla^2_{\m{xy}}g(\m{x},\m{y};\zeta_{N'+1})\\
% &\Big[\frac{N}{\ell_{g,1}}\prod\limits_{n=1}^{N'}\Big(\m{I}-\frac{1}{\ell_{g,1}} \nabla^2_{\m{y}} g(\m{x},\m{y};\zeta_n)\Big)\Big] \nabla_y f(\m{x},\m{y};\xi).
% % &\Big[\frac{N}{\ell_{g,1}}\prod\limits_{n=1}^{N'}\Big(\m{I}-\frac{1}{\ell_{g,1}} \nabla^2_{\m{y}} g(\m{x},\m{y};\zeta_n)\Big)\Big] \nabla_y f(\m{x},\m{y};\xi),
% % &\bar{\nabla}f(\m{x},\m{y})  \approx \nabla_{\m{x}} f(\m{x}, \m{y}, \xi)-\nabla^2_{\m{xy}}g(\m{x},\m{y};\zeta_{N'+1})\cdot\\
% % &\Big[\frac{N}{\ell_{g,1}}\prod\limits_{n=1}^{N'}\Big(\m{I}-\frac{1}{\ell_{g,1}} \nabla^2_{\m{y}} g(\m{x},\m{y};\zeta_n)\Big)\Big] \nabla_y f(\m{x},\m{y};\xi),
% \end{align}
% \end{subequations}
% Here, $N'$ is drawn from $\{0,  \ldots, N-1\}$ uniformly at random (UAR), $\{\zeta_{1}, \ldots,\zeta_{N'}\}$ are i.i.d.~samples. 
% It has been shown in \citep{ghadimi2018approximation,hong2020two} that using \eqref{eq.inverse-estimator}, the inverse Hessian estimation bias $[\nabla_{\m{y}}^{2}g]^{-1}$ exponentially decreases with the number of samples $N$. It should be mentioned that the above approximation is not the only construction, and bilevel optimization can accommodate other forms of gradient surrogates~\citep{ji2021bilevel}.  However, in our case, problem is more daunting as the Hessian is distributed across users and classical Hessian approximations are not applicable.
% \begin{align}
% \bar{\m{h}}^{\texttt{dir}}(\m{x},\m{y})=\mb{E}_{\xi}[\m{h}^{\texttt{dir}}(\m{x},\m{y})], \bar{\m{h}}^{\texttt{indir}}(\m{x},\m{y})=\mb{E}_{\xi} \m{h}^{\texttt{indir}}(\m{x},\m{y}),     
% \end{align}
%, and $\prod\limits_{n=1}^{0}\big(\m{I}-\frac{1}{\ell_{g,1}} \nabla^2_{\m{y}} g(\m{x},\m{y};\zeta_n)\big)=:\m{I}$
\subsection{Outer Optimizer: \fedout}\label{sec:fedout}
%
\input{sec/fedout}
\input{sec/fedihgp}

This section presents the outer optimizer \fedout, formally described in Algorithm~\ref{alg:fedout}. As a subroutine of \fedblo (see Line 9, Algorithm~\ref{alg:fednest}), at each round $k=0,\ldots,K-1$, \fedout takes the most recent global outer model $\x^k$ together the updated (by \fedinn) global inner model $\y^{k+1}$ and produces an update $\x^{k+1}$. To lighten notation, for a round $k$, denote the function's input as $(\m{x}, \m{y}^+)$ (instead of $(\x^k,\y^{k+1})$) and the output as $\m{x}^+$ (instead of $\x^{k+1}$).
%suppose at each round $k$, when calling \fedout the server has inner \& outer models $(\m{x}, \m{y}^+):=(\x^k,\y^{k+1})$ and }. Also, let $\mc{S}$ denote the set of clients $\mc{S}$. 
%\ct{Is it necessary here that the participating set of clients $\mc{S}$ is $\{1,\ldots,m$ or can be subset?}
For each client $i\in \mathcal{S}$, \fedout uses   stochastic approximations of $\bar{\nabla}^{\texttt{I}} f_i(\m{x},\m{y}^+)$ and $\bar{\nabla}^{\texttt{D}}f_i(\m{x},\m{y}^+)$, which we call  $\m{h}_i^{\texttt{I}}(\m{x}, \m{y}^+)$ and $\m{h}_i^{\texttt{D}}(\m{x}, \m{y}^+)$, respectively.  The specific choice of these approximations (see Line 5) is critical and is discussed in detail later in this section. Before that, we explain how each client uses these proxies to form  local updates of the outer variable.
%Specifically, it sets  $\m{h}_i^{\texttt{D}}(\m{x}, \m{y}^+)=\nabla_{\x}  f_i(\x,\y^+;\xi_i)$ and $\m{h}_i^{\texttt{I}}(\m{x}, \m{y}^+)=\nabla^2_{\m{xy}}g_i(\m{x},\m{y}^+;{\zeta}_{i})\m{p}_N$
%let $\m{h}_i^{\texttt{I}}(\m{x}, \m{y})$ and $\m{h}_i^{\texttt{D}}(\m{x}, \m{y})$ denote the stochastic approximations of $\bar{\nabla}^{\texttt{I}} f_i(\m{x},\m{y})$ and $\bar{\nabla}^{\texttt{D}}f_i(\m{x},\m{y})$, respectively. 
In each round, starting from a common global model $\m{x}_{i,0}=\m{x}$, each client $i$ performs $\tau_i$ local steps (in parallel):
%\begin{subequations}\label{eqn:update:fedout}
\begin{align}\label{eqn:update1:fedout}
\m{x}_{i,\nu +1} = \m{x}_{i,\nu }-\alpha_i\m{h}_{i,\nu },
\end{align}
and then the server aggregates local models via $\m{x}^+=|\mc{S}|^{-1} \sum_{i\in \mc{S}} \m{x}_{i,\tau_i}$. Here, $\alpha_i \in (0,\alpha]$ is the local stepsize, 
\begin{equation}\label{eqn:hyper:estim}
\begin{aligned}
\m{h}_{i,\nu }:=&\m{h}^{\texttt{I}}(\m{x},\m{y}^{+})+  \m{h}^{\texttt{D}}(\m{x},\m{y}^{+})\\
&-\m{h}_i^{\texttt{D}}(\m{x},\m{y}^{+})+\m{h}_i^{\texttt{D}}(\m{x}_{i,\nu },\m{y}^{+})\,,
\end{aligned}
\end{equation}
$\m{h}^{\texttt{I}}(\m{x},\m{y}) := |\mc{S}|^{-1}\sum_{i\in\mathcal{S}} \m{h}_i^{\texttt{I}} (\m{x},\m{y})$, and $\m{h}^{\texttt{D}}(\m{x},\m{y}) := |\mc{S}|^{-1}\sum_{i\in\mathcal{S}} \m{h}_i^{\texttt{D}} (\m{x},\m{y})$. 
%and \left(\m{h}_i^{\texttt{D}}(\m{x}, \m{y}^+)-\m{h}_i^{\texttt{I}}(\m{x}, \m{y}^+)\right).$

The key features of updates~\eqref{eqn:update1:fedout}--\eqref{eqn:hyper:estim} are exploiting past gradients (variance reduction) to account for objective heterogeneity. Indeed,
%and using client-specific stepsize $\alpha_i$ to tackle systems heterogeneity. Next, we discuss these features in detail.}
%objective heterogeneity
%\textbf{Outer Local SGD:} 
the ideal update in \fedout would perform the update $\m{x}_{i,\nu +1} =\m{x}_{i,\nu }-\alpha_i\big(\m{h}^{\texttt{I}}(\m{x}_{i,\nu },\m{y}^{+})+ \m{h}^{\texttt{D}}(\m{x}_{i,\nu },\m{y}^{+})\big)$ using the global gradient estimates. But this requires each client $i$ to have access to both direct and indirect gradients of all other clients--which it does not, since clients do not communicate between rounds. To overcome this issue, each client $i$ uses global gradient estimates, i.e., $ \m{h}^{\texttt{I}}(\m{x},\m{y}^{+})+\m{h}^{\texttt{D}}(\m{x},\m{y}^{+})$ from the beginning of each round as a guiding direction in its local update rule. However, since both $\m{h}^{\texttt{D}}$ and $\m{h}^{\texttt{I}}$ are computed at a previous  $(\m{x},\m{y}^{+})$, client $i$ makes a correction by subtracting off the stale direct gradient estimate $\m{h}_i^{\texttt{D}}(\m{x},\m{y}^{+})$ and adding its own \emph{local} estimate $\m{h}_i^{\texttt{D}}(\m{x}_{i,\nu },\m{y}^{+})$. Our local update rule in Step~11 of Algorithm~\ref{alg:fedout} is precisely of this form, i.e.,  $\m{h}_{i,\nu }$ approximates
%an inexact version of 
$\m{h}^{\texttt{I}}(\m{x}_{i,\nu },\m{y}^{+})+ \m{h}^{\texttt{D}}(\m{x}_{i,\nu },\m{y}^{+})$
%. In particular, we approximate the ideal $\m{h}^{\texttt{I}}(\m{x}_{i,\nu },\m{y}^{+})+ \m{h}^{\texttt{D}}(\m{x}_{i,\nu },\m{y}^{+})$ 
via \eqref{eqn:hyper:estim}. Note here that the described local correction of \fedout only applies to the direct gradient component (the indirect component would require global Hessian information). An alterantive approach leading to \lfedblo is discussed in Section \ref{light blo}.

%While \fedout does not utilize local indirect gradients, we overcome this issue by proposing the more practical algorithm \lfedblo as described in Section \ref{light blo}.

\noindent\textbf{\fedout applied to special nested problems.} Algorithm~\ref{alg:fedout} naturally allows the use of other optimizers for minimax \& compositional optimization. For example, in the minimax problem~\eqref{fedminmax:prob}, the bilevel gradient components are $\nabla^{\texttt{D}} f_i(\m{x},\m{y}^*(\m{x}))=\nabla_{\m{x}}f_i\left(\m{x},\m{y}^*(\m{x})\right)$ and $\nabla^{\texttt{I}} f_i(\m{x},\m{y}^*(\m{x}))=0$ for all $i \in\mc{S}$. Hence, the hypergradient estimate \eqref{eqn:hyper:estim} reduces to 
\begin{equation}\label{eqn:hyper:estim:minmax}
 \m{h}_{i,\nu } = \m{h}^{\texttt{D}}(\m{x},\m{y}^{+})-\m{h}_i^{\texttt{D}}(\m{x},\m{y}^{+})+\m{h}_i^{\texttt{D}}(\m{x}_{i,\nu },\m{y}^{+}). 
\end{equation}
%To the best of our knowledge,  ... 
For the compositional problem~\eqref{fedcompos:prob2}, Hessian becomes the identity matrix, the direct gradient is the zero vector, and  $\nabla_{\m{xy}}g(\m{x},\m{y})=- (1/m)\sum_{i=1}^m\nabla \m{r}_i(\m{x})^{\top}$. Hence, $\m{h}_i= \ell_{g,1}\nabla  \m{r}_i(\m{x})^{\top} \m{p}_{0}$ for all $i \in\mc{S}$. 

%This together with \eqref{main_grad:decom} and \eqref{eq.inverse-estimator.b} gives which implies that $\nabla^{\texttt{D}} f_i(\m{x},\m{y}^*(\m{x}))=0$ and $\nabla^{\texttt{I}} f_i(\m{x},\m{y}^*(\m{x}))= (\frac{1}{m}\sum_{i=1}^m\nabla h_i(\m{x}))^{\top}\nabla_\m{y} f_i(\m{y}^\star(\m{x}))$ for all $i \in\mc{S}$.

More details on these special cases are provided in Appendices~\ref{sec:app:minmax}~and~\ref{sec:app:compos}.   

\noindent\textbf{Indirect gradient estimation \& \fedhess.} Here, we aim to address one of the key challenges in nested FL: inverse Hessian gradient product.  Note from \eqref{eq.inverse-estimator.b} that the proposed stochastic approximation of the indirect gradient involves in a nonlinear way the \emph{global} Hessian, which is \emph{not} available at the client. To get around this, we use a client sampling strategy and recursive reformulation of \eqref{eq.inverse-estimator.b} so that $\bar{\nabla}^{\texttt{I}}f_i(\m{x},\m{y})$ can be estimated in an efficient federated manner. In particular, given $N \in \mb{N}$, we select $N' \in \{0 \ldots, N-1\}$ and $\mc{S}_0, \ldots, \mc{S}_{ N'} \in \mc{S}$ UAR. For all $i \in \mc{S}$, we then define
\begin{subequations}
\begin{equation}\label{eq:grad:est} 
\begin{aligned}
&\m{h}^{\texttt{I}}_i(\m{x},\m{y}) =-\nabla^2_{\m{xy}}g_i(\m{x},\m{y};\zeta_{i}) \m{p}_{N'},
\end{aligned}    
\end{equation}
where $\m{p}_{N'}=|\mc{S}_0|^{-1}\wh{\m{H}}_\m{y} \sum_{i\in\mc{S}_0} \nabla_\m{y} f_i(\m{x}, \m{y};\xi_{i,0})$ and $\wh{\m{H}}_\m{y}$ is the approximate inverse Hessian:
\begin{align}
\frac{ N}{\ell_{g,1}} \prod_{n=1}^{N'} \Big (\m{I} - \frac{1}{ \ell_{g,1}  |\mc{S}_n|} \sum_{i=1}^{|\mc{S}_n|} \nabla_{\m{y}}^2 g_i(\m{x},\m{y}; \zeta_{i,n}) \Big).
\label{eq:hessinv:est}
\end{align}
\end{subequations}
The subroutine \fedhess provides a recursive strategy to compute $\m{p}_{N'}$  and \fedout multiplies $\m{p}_{N'}$ 
with the Jacobian to drive an indirect gradient estimate. Importantly, {these approximations require only matrix-vector products and vector communications.}

\begin{lemma}\label{lem:neum:bias}
Under Assumptions~\ref{assu:f} and \ref{assu:bound:var}, the approximate inverse Hessian $\wh{\m{H}}_\m{y}$ defined in \eqref{eq:hessinv:est} satisfies the following for any $\x$ and $\y$:
\begin{align}
\nonumber 
\left\|\left[\nabla^2_{\m{y}} g (\m{x}, \m{y})\right]^{-1} - \mb{E}_{\mc{W}}[\wh{\m{H}}_{\m{y}}]\right\| &\le \frac{1}{\mu_g} \left(\frac{\kappa_g-1}{\kappa_g} \right)^N,\\
\mb{E}_{\mc{W}}\left[\left\|\left[\nabla^{2}_{\m{y}} g (\m{x}, \m{y})\right]^{-1}-\wh{\m{H}}_{\m{y}}\right\|\right] &\le \frac{2}{\mu_g}. \label{Hessian_Invs_ineq}
\end{align}
Here, $\mc{W}:=\left\{\mc{S}_n, \xi_{i},\zeta_{i}, \xi_{i,0}, \zeta_{i,n} \mid i \in \mc{S}_n, ~~~0\leq n\leq  N' \right\}$. Further, for all $~i \in \mc{S}$, $\m{h}_i^{\texttt{I}}(\m{x},\m{y})$ defined in \eqref{eq:grad:est} satisfies
\begin{align}
\left\| \mb{E}_{\mc{W}} \left[\m{h}_i^{\texttt{I}}(\m{x},\m{y})\right]- \bar{\nabla}^{\texttt{I}} f_i(\m{x},\m{y}) \right\|&\leq b, 
\end{align}
where $b:= \kappa_g\ell_{f,1}\big( (\kappa_g-1)/\kappa_g \big)^{N}$.
\end{lemma}

\subsection{Inner Optimizer: \fedinn}\label{sec:fedinn}


In FL, each client performs multiple local training steps in isolation on its own data (using for example SGD) before communicating with the server. Due to such local steps, \fedavg  suffers from a \textit{client-drift} effect under objective heterogeneity; that is, the local iterates of each client drift-off towards the minimum of their own local function. In turn, this can  lead to convergence to a point different from the  global optimum $\y^*(\x)$ of the inner problem; e.g., see \citep{mitra2021linear}. This behavior is particularly undesirable in a nested optimization setting since it directly affects the outer optimization; see, e.g. \citep[Section~7]{liu2021investigating}.  

In light of this observation, we build on the recently proposed \textsc{FedLin}~\citep{mitra2021linear} which improves \textsc{FedSVRG}~\citep{konevcny2016federated} to solve the inner problem; see Algorithm~\ref{alg:fedinn}. For each $i\in \mc{S}$, let  $\m{q}_i(\m{x}, \m{y})$ denote an unbiased estimate of the gradient $\nabla_{\m{y}} g_i(\m{x},\m{y})$. In each round, starting from a common global model $\m{y}$, each client $i$ performs $\tau_i$ local SVRG-type training steps in parallel: 
% \begin{equation*}
$\m{y}_{i,\nu +1} = \m{y}_{i,\nu }-\beta_i\m{q}_{i,\nu },$  
% \end{equation*}
where $\m{q}_{i,\nu }:= \m{q}_i(\m{x},\m{y}_{i,\nu })-\m{q}_i(\m{x},\m{y})+\m{q}(\m{x},\m{y})$, $\beta_i \in (0,\beta]$ is the local inner stepsize, and $\m{q}(\m{x},\m{y}) := |\mc{S}|^{-1}\sum_{i\in\mathcal{S}} \m{q}_i(\m{x},\m{y})$. We note that for the optimization problems \eqref{fedblo:prob}, \eqref{fedminmax:prob}, and \eqref{fedcompos:prob2}, $\m{q}_i(\m{x},\m{y}_{i,\nu })$ is equal to $\nabla_\m{y} g_i(\m{x}, \m{y}_{i,\nu };\zeta_{i,\nu })$, $-\nabla_\m{y} f_i(\m{x}, \m{y}_{i,\nu };\xi_{i,\nu })$, and $\m{y}_{i,\nu }-\m{r}_i(\m{x};\zeta_{i,\nu })$, respectively; see  Appendices~\ref{sec:app:bilevel}--\ref{sec:app:compos}.
\input{sec/fedinn}




%\noindent\textbf{Simplified \fedout.} 
\subsection{Light-\fedblo: Communication Efficiency via Local Hypergradients}\label{light blo}
%\textbf{Communication efficiency of \fedblo:}
 Each \fednest epoch $k$ requires $2T+N+3$ communication rounds as follows: $2T$ rounds for SVRG of \fedinn, 
%due to $T$ rounds of SVRG 
$N$ iterations for inverse Hessian approximation within \fedhess and $3$ additional aggregations. Note that, these are vector communications and we fully avoid Hessian communication. 
%Our \fedout\& \fedhess use global inverse Hessian and gradient estimates to tackle objective heterogeneity and to establish provable convergence guarantees without stringent assumptions. 
In Appendix~\ref{sec:simp:algs}, we also propose simplified variants of \fedout and \fedhess, {which are tailored to homogeneous or  high-dimensional FL settings}. These algorithms can then either use \textit{local} Jacobian / inverse Hessian or their approximation, and can use either SVRG or SGD. 

\noindent\textbf{Light-\fedblo:} Specifically, we propose \lfedblo where each client runs IHGP locally.  This reduces the number of rounds to $T+1$, saving $T+N+2$ rounds (see experiments in Section \ref{sec:numerics} for performance comparison and Appendix~\ref{sec:simp:algs} for further discussion.)

==> FedNest_ _/sec/conc.tex <==
%\vspace{-.4cm}
\section{Conclusions}\label{sec:conc}
We presented a new class of federated algorithms for solving general nested stochastic optimization spanning bilevel and \minmax~problems. \fednest runs a variant of federated SVRG on inner \& outer variables in an alternating fashion. We established provable convergence rates for \fednest under arbitrary client heterogeneity and introduced variations for min-max and compositional problems and for improved communication efficiency (\lfedblo). We showed that, to achieve an $\epsilon$-stationary point of the nested problem, \fednest requires $O(\epsilon^{-2})$ samples in total, which matches the complexity of the non-federated nested algorithms in the literature. 
%objective and systems

\vspace{-5pt}
\section*{Acknowledgements}\vspace{-5pt}
Davoud Ataee Tarzanagh was supported by ARO YIP award W911NF1910027 and NSF CAREER award CCF-1845076. Christos Thrampoulidis was supported by NSF Grant Numbers CCF-2009030 and HDR-1934641, and an NSERC Discovery Grant. Mingchen Li and Samet Oymak were supported by the NSF CAREER award CCF-2046816, Google Research Scholar award, and ARO grant W911NF2110312.

==> FedNest_ _/sec/fedihgp.tex <==
\begin{algorithm}[t]
  \caption{$\m{p}_{N'}=~\pmb{\fedhess}~(\m{x}, \m{y}^+,N)$: Federated approximation of inverse-Hessian-gradient product}
\begin{algorithmic}[1]
%\For{$t=T-1,...,0$}
\State Select $ N'\in \{0, \dots, N-1\}$ UAR.
\State Select $\mc{S}_0 \in \mc{S}$ UAR.
%\State If $N'=0$ 
  \For{$i \in \mc{S}_0$ \textbf{in parallel}} 
 \State $\m{p}_{i,0} =\nabla_\m{y} f_i(\m{x}, \m{y}^+; \xi_{i,0})$
 \EndFor
 \State $ \m{p}_0 = \frac{N}{\ell_{g,1}}  |\mc{S}_0|^{-1}\sum_{i\in\mathcal{S}_0} \m{p}_{i,0}$  %\hspace{.5cm}\texttt{\#communication}  
\If{$N'=0$}
\State  Return $\m{p}_{N'}$
\EndIf
%  \State{{\color{blue} Option~I (Local Inverse):} 
%  \State Select $\mc{S}_{ N'} \in \mc{S}$ UAR.}
%   		\For {$i \in \mc{S}_{N'}$ \textbf{in parallel}} 
% 		 \State $\m{p}_{i,N'} = \prod\limits_{n=1}^{N'} \big(\m{I}-\frac{1}{\ell_{g,1}}\nabla^2_y g_i(\m{x}, \m{y}^+;{\zeta}_{i,n})\big)\m{p}_{0}$% \Comment{$\m{X}_{i,j} := \nabla^2_y g_i(\m{x}, \m{y}^+;\xi_j)$}
% 	   \EndFor
% 	   \State $\m{p}_{N'}= |\mc{S}_{N'}|^{-1}\sum_{i\in\mc{S}_{N'}} \m{p}_{i,N'}$ 
%\State{{\color{blue} Option~II (Global Inverse):}}
\State Select $\mc{S}_1, \ldots, \mc{S}_{ N'} \in \mc{S}$ UAR.
\For{$n=1,\ldots, N'$}
 	   % \State Choose $N' \in \{0,\ldots,N-1\}$ randomly and 
	%	\For {$i \in \mc{S}$ \textbf{in parallel}} 
		\For {$i \in \mc{S}_n$ \textbf{in parallel}} 
		 \State $\m{p}_{i,n} = \left(\m{I}-\frac{1}{\ell_{g,1}}\nabla^2_\m{y} g_i(\m{x}, \m{y}^+;{\zeta}_{i,n})\right)\m{p}_{n-1}$% \Comment{$\m{X}_{i,j} := \nabla^2_y g_i(\m{x}, \m{y}^+;\xi_j)$}
	   \EndFor
	   \State $\m{p}_{n}=|\mc{S}_n|^{-1}\sum_{i\in\mc{S}_n} \m{p}_{i,n}$ %\hspace{.5cm}\texttt{\#communication}  
	   %\Else 
 	   %\State $\m{p}_{i}^{k,t}=\m{p}^{k,t+1}-\beta_i \nabla_\m{y}^+^2  g_i (\m{x},\m{y}^+)\m{p}^{k,t+1}$~~ 
	   %\EndFor
	%	\State $\m{p}^{k,t}= 1/m\sum_{i\in\mathcal{S}} \m{p}_{i}^t$
	%	\State { $\m{p}^k=\sum_{t=0}^{T-1}\m{p}^{k,t}$}
		\EndFor
%\State  Set $\m{p}_{N}= \frac{N}{\ell_{g,1}} \m{p}_{N'}$. Return $\m{p}_N$		
\end{algorithmic}\label{fedihgp_algo}
\end{algorithm}

%\ct{Should $\mathbf{p}_0$ change to use local iterates $x_{i,\ell}$ for OPTION 1? At least, to agree with $h_{i}(x_{i,\ell},y)$.}

==> FedNest_ _/sec/fedinn.tex <==
\begin{algorithm}[t]
\caption{$ \m{y}^+~=~\pmb{\fedinn}~(\m{x},\m{y},\beta$) 
%for stochastic \colorbox{cyan!30}{bilevel (\func$\gets$)}, \colorbox{green!30}{minimax (\func$\gets$)}, and \colorbox{magenta!30}{compositional (\func$\gets$)} problems
}
\label{alg:fedinn}
\begin{algorithmic}[1]
%\For{$t\in(T]$} 
%Set query function 
\State $\funcin_i(\cdot)\gets$ \colorbox{cyan!30}{$\nabla_\m{y} g_i(\m{x},\cdot)$~\text{(bilevel)}},\colorbox{green!30}{$-\nabla_\m{y} f_i(\m{x},\cdot)$~\text{(minimax)}}
%\colorbox{magenta!30}{$-h_i(\cdot)$~\text{(composite)}},\\
%\hspace{37pt}
%\funcin_i\gets 
 \State $\m{y}_{i,0}=\m{y}$ and $\beta_i \in (0,\beta]$
  \For{$i \in \mc{S}$ \textbf{in parallel}} 
 \State $\m{q}_i=\funcin_i(\m{y};  \zeta_{i})$
%\State \colorbox{green!30}{$\m{q}_i=-\nabla_\m{y} f_i(\m{x}, \m{y};  \xi_{i})$}
% \State \colorbox{magenta!30}{$\m{q}_i=-h_i(\m{x}; \zeta_{i})$}
 \EndFor
 \State $\m{q}=|\mathcal{S}|^{-1}\sum_{i\in\mathcal{S}}\m{q}_i$ %\hspace{1.5cm}\texttt{\#communication}  
 \For {$i \in \mc{S}$ \textbf{in parallel}} 
 %\State Choose $\beta_i \in (0, \beta)$
\For {$\nu=0,\ldots,\tau_i-1$} 
%\vspace{2mm}
\State $\m{q}_{i,\nu }=\funcin_i(\m{y}_{i,\nu };\zeta_{i,\nu })-\funcin_i(\m{y};\zeta_{i,\nu })+\m{q}$
%\State \colorbox{green!30}{$ \m{q}_{i,\nu }=-\nabla_\m{y} f_i(\m{x}, \m{y}_{i,\nu };\xi_{i,\nu })+\nabla_\m{y} f_i(\m{x}, \m{y};\xi_{i,\nu })$}
%\State \colorbox{magenta!30}{$ \m{q}_{i,\nu }=h_i(\m{x}_{i,\nu };\zeta_{i,\nu })-h_i(\m{x};\zeta_{i,\nu })$}
\State $\m{y}_{i,\nu +1}= \m{y}_{i,\nu }-\beta_i\m{q}_{i,\nu }$
\EndFor
\EndFor
\State $\m{y}^{+}=|\mathcal{S}|^{-1}\sum_{i\in\mathcal{S}}\m{y}_{i,\tau_i}$ %\hspace{1cm}\texttt{\#communication}  
%\EndFor
\end{algorithmic}
\end{algorithm}
% \begin{algorithm}[t]
% \caption{$ \m{y}^T ~=~\pmb{\fedinn}~(\m{x},\m{y}^{0},T,\beta$) for stochastic \colorbox{red!30}{bilevel} and \colorbox{green!30}{minimax} problems}
% \label{algo:svrg}
% \begin{algorithmic}[1]
% %\For{$t\in(T]$} 
%   \For{$i \in \mc{S}$ \textbf{in parallel}} 
%  \State \colorbox{red!30}{$\m{q}^t_i=\nabla_y g_i(\m{x}, \m{y}^{t};  \zeta_{i}^t)$}
%  \State \colorbox{green!30}{$\m{q}^t_i=-\nabla_y f_i(\m{x}, \m{y}^{t};  \xi_{i}^t)$}
%  \EndFor
%  \State $\m{q}^t=|\mathcal{S}|^{-1}\sum_{i\in\mathcal{S}}\m{q}^t_i$
%  \State $\m{y}^t_{i,0}=\m{y}^t$
%  \For {$i \in \mc{S}$ \textbf{in parallel}} 
%  %\State Choose $\beta_i \in (0, \beta)$
% \For {$\ell=0,\ldots,\tau_i-1$} 
% %\vspace{2mm}
% \State \colorbox{red!30}{$\m{q}_{i,\nu }^t=\nabla_y g_i(\m{x}, \m{y}^t_{i,\nu };\zeta_{i,\nu }^t)-\nabla_y g_i(\m{x}, \m{y}^{t};\zeta_{i,\nu }^t)$}
% \State \colorbox{green!30}{$ \m{q}_{i,\nu }^t=-\nabla_y f_i(\m{x}, \m{y}^t_{i,\nu };\xi_{i,\nu }^t)+\nabla_y f_i(\m{x}, \m{y}^{t};\xi_{i,\nu }^t)$}
% \State $\m{y}^{t}_{i,\nu +1} \gets \m{y}^{t}_{i,\nu }-\beta_i (\m{q}_{i,\nu }^t+\m{q}^t)$
% \EndFor
% \EndFor
% \State $\m{y}^{t+1}=|\mathcal{S}|^{-1}\sum_{i\in\mathcal{S}}\m{y}^t_{i,\tau_i}$
% %\EndFor
% \end{algorithmic}
% \end{algorithm}

==> FedNest_ _/sec/fednest.tex <==
%\begin{minipage}[t]{.3\textwidth}
%\end{minipage}
%\begin{wrapfigure}{L}{0.47\textwidth}
%\begin{minipage}{0.47\textwidth}
 %   \vspace{-8mm}
\begin{algorithm}[t]
\caption{\pmb{\fedblo}}
\label{alg:fedblo}
\begin{algorithmic}[1]
\State \textbf{Inputs:} $K,T \in \mb{N}$;~~$(\m{x}^0, \m{y}^0)\in \mb{R}^{d_1+d_{2}}$;~~\textbf{\fedinn},\\
\hspace{33pt}\textbf{\fedout} with stepsizes $\{(\alpha^k, \beta^k)\}_{k=0}^{K-1}$
%	    \While{not converged}
\For{$k = 0, \cdots, K-1$}
\State $\m{y}^{k,0}=\m{y}^k$
\For{$t = 0, \cdots, T-1$}
\State $\m{y}^{k,t+1}=\pmb{\fedinn}\left(\m{x}^k,\m{y}^{k,t},\beta^k \right)$~~~
\EndFor
\State $\m{y}^{k+1}=\m{y}^{k,T}$
\State $\m{x}^{k+1}=\pmb{\fedout}\left(\m{x}^k,\m{y}^{k+1}, \alpha^k \right)$
%\State $\m{y}^{k+1}= 
\EndFor
%\EndWhilexx
\end{algorithmic}\label{alg:fednest}
\end{algorithm}
%\vspace{-5mm}
%\end{minipage}
%\end{wrapfigure}
%

==> FedNest_ _/sec/fedout.tex <==
\begin{algorithm}[t]
\caption{$\m{x}^{+} ~=~\pmb{\fedout}~(\m{x}, \m{y}^+, \alpha)$ for stochastic \colorbox{cyan!30}{bilevel} and  \colorbox{green!30}{minimax} problems
%
%\ct{Maybe change input to $\y^{+}$ for consistency with section?}
%,
%and \colorbox{magenta!30}{compositional} 
} %\colorbox{purple!30}{SVRG}}
\begin{algorithmic}[1]
\State $\funco_i(\cdot)\gets \nabla_\m{x} f_i(\cdot,\m{y}^+;\cdot)$ %(bilevel \& min-max), 
%\\
%\hspace{30pt}\colorbox{magenta!30}{$\gets \nabla_\m{x} h_i(.) \nabla_\m{y}^+ f_i(.)$~(compositional)}   
%\colorbox{cyan!30}{$\nabla_\m{y}^+ f_i(\cdot)$~\text{(bilevel)}}, \colorbox{green!30}{$-\nabla_\m{y}^+ f_i(\cdot)$~\text{(min-max)}},\\ \hspace{35pt}\colorbox{magenta!30}{$-h_i(\cdot)$~\text{(composite)}}%\func_i\gets 
 \State $\m{x}_{i,0}=\m{x}$ and $\alpha_i \in (0,\alpha]$
\State \colorbox{cyan!30}{Choose $N \in \mb{N}$ and set $ \m{p}_{N^{'}}=~\pmb{\fedhess}~(\m{x}, \m{y}^+,N)$}
 \For{$i \in \mc{S}$ \textbf{in parallel}} 
 \State \colorbox{cyan!30}{$\m{h}_i= \funco_i(\m{x};\xi_{i})-\nabla^2_{\m{xy}}g_i(\m{x},\m{y}^+;{\zeta}_{i})
 \m{p}_{N^{'}}$}
% \State \colorbox{green!30}{$\m{h}_i=\funco_i(\m{x};  \xi_{i})$},  \colorbox{magenta!30}{$\m{h}_i= \nabla h_i(\m{x};  \zeta_{i}) \nabla f_i(\m{y}^+;  \xi_{i})$}
  \State \colorbox{green!30}{$\m{h}_i=\funco_i(\m{x};  \xi_{i})$}
 %  \State   \colorbox{magenta!30}{$\m{h}_i= \nabla^2_{\m{xy}}g_i(\m{x},\m{y}^+;{\zeta}_{i})
 %\m{p}_0$}
 \EndFor
 \State $\m{h}=|\mathcal{S}|^{-1}\sum_{i\in\mathcal{S}}\m{h}_i$ %\hspace{1.5cm}\texttt{\#communication}    
 \For {$i \in \mc{S}$ \textbf{in parallel}} 
\For {$\nu= 0,\ldots,\tau_i-1$} 
 %\State Choose $\beta_i \in (0, \beta)$
% \For {$i \in \mc{S}$ \textbf{in parallel}} 
 \State%\colorbox{cyan!30}{
$\m{h}_{i,\nu }=\funco_i(\m{x}_{i,\nu }; \xi_{i,\nu })-\funco_i(\m{x}; \xi_{i,\nu })+\m{h}$
%\colorbox{magenta!30}{$\m{h}_{i,\nu }= \nabla h_i(\m{x}_{i,\nu };  \zeta_{i}) \nabla f_i(\m{y}^+_{i,\nu };  \xi_{i,\nu })+ \nabla h_i(\m{x};  \zeta_{i}) \nabla f_i(\m{y}^+_{i,\nu };  \xi_{i,\nu })$
%}
 %}%\colorbox{purple!30}{SVRG}
% \State \colorbox{red!30}{$ \m{h}_{i,\nu }= \nabla_{\m{x}} f_i(\m{x}, \m{y}^+^*(\m{x}))-\nabla^2_{\m{xy}}g_i(\m{x},\m{y}^+^*(\m{x}))
% \m{p}_N $}-%\colorbox{purple!30}{SVRG}
% \State\colorbox{green!30}{$\m{h}_{i,\nu }=\nabla_{\m{x}} f_i(\m{x}_{i,\nu }, \m{y}^+; \xi_{i,\nu })-\nabla_{\m{x}} f_i(\m{x}, \m{y}^+; \xi_{i,\nu })$}%\colorbox{purple!30}{SVRG}
%\State \colorbox{magenta!30}{$\m{h}_{i,\nu }=-\nabla_y f_i(\m{x}, \m{y}^+;  \xi_{i})$}
 %\State \colorbox{magenta!30}{$\m{h}_i=\nabla h_i(\m{x}_{i,\nu };  \zeta_{i,\nu }) \nabla f_i(\m{y}^+_{i,\nu };  \xi_{i,\nu })-\nabla h_i(\m{x}; \zeta_{i,\nu }) \nabla f_i(\m{y}^+;  \xi_{i,\nu })$}
 %~~\Comment{via automatic differentiation}
% \State  $\m{H}_i^{k+1} = \m{H}_i^k + \pi_1 \m{S}_i^k$ and $\m{J}_i^{k+1} = \m{J}_i^k + \pi_2\m{W}_i^k$;
% %\Stae Send $\nabla f_i(x^k)$,\; $\mS_i^k \eqdef \cC_i^k(\nabla^2 f_i(x^k) - \mH_i^k)$ and $l_i^k \eqdef \|\mH_i^k - \nabla^2 f_i(x^k)\|_{\rm F}$ to the server
%\State  $\m{x}^{+}=1/m\sum_{i\in\mathcal{S}}\m{x}_{i}$
 \State  $ \m{x}_{i,\nu +1}= \m{x}_{i,\nu }- \alpha_i\m{h}_{i,\nu }$%~~\Comment{via automatic
  \EndFor
\EndFor
\State $\m{x}^{+}=|\mc{S}|^{-1}\sum_{i\in \mc{S}} \m{x}_{i,\tau_i}$ %\hspace{1cm}\texttt{\#communication}  
% \EndFor
\end{algorithmic}
\label{alg:fedout}
\end{algorithm}







% Estimator~\eqref{eq.inverse-estimator} is not time and memory efficient to compute in  federated setting due to the summation inverse in \eqref{eqn:grad:y}. Besides, in 

%It can be easily seen that the above procedure gives an estimate of $\tilde{\nabla}f(\m{x},\m{y})$ with three rounds of vector communication with the server.


% \begin{figure*}
%  \begin{subfigure}{.47\textwidth}

%  \end{subfigure}
%   \hspace*{0.03in}
%  \begin{subfigure}{.5\textwidth}
%   \tiny{
% \begin{algorithm}[H]
%   \caption*{$\m{x}^{+} ~=~\pmb{\fedout}~(\m{x}, \m{y}, \alpha,N$ }
% \begin{algorithmic}[1]
% %\For{$t=T-1,...,0$}
% \State Select $ N'\in \{1, \dots, N\}$ and $\mc{S}_0, \ldots, \mc{S}_{ N'+1} \in \mc{S}$ uniformly at random.
%   \For{$i \in \mc{S}_0$ \textbf{in parallel}} 
%  \State Compute $\nabla_y f_i(\m{x}, \m{y}; \xi_{i,n})$
%  \EndFor
%  \State $ \m{p}_0 \leftarrow 1/|\mc{S}_0|\sum_{i\in\mathcal{S}_0} \nabla_y f_i(\m{x}, \m{y}; \xi_{i,n})$ 
%  	%	\State $\m{p}_{i,0}\leftarrow \m{p}$
%  		 \For{$n=1,\ldots, N'$}
%  	   % \State Choose $N' \in \{0,\ldots,N-1\}$ randomly and 
% 	%	\For {$i \in \mc{S}$ \textbf{in parallel}} 
% 		\For {$i \in \mc{S}_n$ \textbf{in parallel}} 
% 		 \State $\m{p}_{i,n} \leftarrow (\m{I}-\frac{1}{\ell_{g,1}}\nabla^2_y g_i(\m{x}, \m{y};{\zeta}_{i,n}))\m{p}_{n-1}$% \Comment{$\m{X}_{i,j} := \nabla^2_y g_i(\m{x}, \m{y};\xi_j)$}
% 	   \EndFor
% 	   \State $\m{p}_{n}\leftarrow 1/|\mc{S}_n|\sum_{i\in|\mc{S}_n|} \m{p}_{i,n}$
% 	   %\Else 
%  	   %\State $\m{p}_{i}^{k,t}=\m{p}^{k,t+1}-\beta_i \nabla_\m{y}^2  g_i (\m{x},\m{y})\m{p}^{k,t+1}$~~ 
% 	   %\EndFor
% 	%	\State $\m{p}^{k,t}= 1/m\sum_{i\in\mathcal{S}} \m{p}_{i}^t$
% 	%	\State { $\m{p}^k=\sum_{t=0}^{T-1}\m{p}^{k,t}$}
% 		\EndFor
%  	%	\State $\m{p}_{N'}= 1/m\sum_{i\in\mathcal{S}} \m{p}_{i,N'}$ \som{Do we explicitly calculate this, or use HVP (ideal approach)? It should be clarified and we can discuss if needed.}
%  \For {$i \in \mc{S}_{N'+1}$ \textbf{in parallel}} 
%  \State $ \m{x}_{i}= \m{x}_i- \alpha (\nabla_{\m{x}} f_i(\m{x}, \m{y}, \xi_{i})- \frac{N}{\ell_{g,1}}\nabla^2_{\m{xy}}g_i(\m{x},\m{y};{\zeta}_{i,N'+1}) \m{p}_{N'}) $%~~\Comment{via automatic differentiation}
% % \State  $\m{H}_i^{k+1} = \m{H}_i^k + \pi_1 \m{S}_i^k$ and $\m{J}_i^{k+1} = \m{J}_i^k + \pi_2\m{W}_i^k$;
% % %\State Send $\nabla f_i(x^k)$,\; $\mS_i^k \eqdef \cC_i^k(\nabla^2 f_i(x^k) - \mH_i^k)$ and $l_i^k \eqdef \|\mH_i^k - \nabla^2 f_i(x^k)\|_{\rm F}$ to the server
% %\State  $\m{x}^{+}=1/m\sum_{i\in\mathcal{S}}\m{x}_{i}$
% \EndFor
% \State  $\m{x}^{+}=1/|\mc{S}_{N'+1}|\sum_{i\in \mc{S}_{N'+1}} \m{x}_{i}$
% % \EndFor
% \end{algorithmic}
% \end{algorithm}
% }
%  \end{subfigure}
%   \vspace*{-0.15in}
% \end{figure*}



% \begin{figure*}
%  \begin{subfigure}{.47\textwidth}
% \begin{algorithm}[H]
%   \caption*{$\m{x}^{+} ~=~\pmb{\fedout}~(\m{x}, \m{y}, \alpha,N$}
% \begin{algorithmic}[1]
% %\For{$t=T-1,...,0$}
% \State Select $ N'\in \{1, \dots, N\}$ and $\mc{S}_0, \ldots, \mc{S}_{ N'+1} \in \mc{S}$ uniformly at random.
%   \For{$i \in \mc{S}_0$ \textbf{in parallel}} 
%  \State Compute $\nabla_y f_i(\m{x}, \m{y}; \xi_{i,n})$
%  \EndFor
%  \State $ \m{p}_0 \leftarrow 1/|\mc{S}_0|\sum_{i\in\mathcal{S}_0} \nabla_y f_i(\m{x}, \m{y}; \xi_{i,n})$ 
%  	%	\State $\m{p}_{i,0}\leftarrow \m{p}$
%  		 \For{$n=1,\ldots, N'$}
%  	   % \State Choose $N' \in \{0,\ldots,N-1\}$ randomly and 
% 	%	\For {$i \in \mc{S}$ \textbf{in parallel}} 
% 		\For {$i \in \mc{S}_n$ \textbf{in parallel}} 
% 		 \State $\m{p}_{i,n} \leftarrow (\m{I}-\frac{1}{\ell_{g,1}}\nabla^2_y g_i(\m{x}, \m{y};{\zeta}_{i,n}))\m{p}_{n-1}$% \Comment{$\m{X}_{i,j} := \nabla^2_y g_i(\m{x}, \m{y};\xi_j)$}
% 	   \EndFor
% 	   \State $\m{p}_{n}\leftarrow 1/|\mc{S}_n|\sum_{i\in|\mc{S}_n|} \m{p}_{i,n}$
% 	   %\Else 
%  	   %\State $\m{p}_{i}^{k,t}=\m{p}^{k,t+1}-\beta_i \nabla_\m{y}^2  g_i (\m{x},\m{y})\m{p}^{k,t+1}$~~ 
% 	   %\EndFor
% 	%	\State $\m{p}^{k,t}= 1/m\sum_{i\in\mathcal{S}} \m{p}_{i}^t$
% 	%	\State { $\m{p}^k=\sum_{t=0}^{T-1}\m{p}^{k,t}$}
% 		\EndFor
%  	%	\State $\m{p}_{N'}= 1/m\sum_{i\in\mathcal{S}} \m{p}_{i,N'}$ \som{Do we explicitly calculate this, or use HVP (ideal approach)? It should be clarified and we can discuss if needed.}
%  \For {$i \in \mc{S}_{N'+1}$ \textbf{in parallel}} 
%  \State $ \m{x}_{i}= \m{x}_i- \alpha (\nabla_{\m{x}} f_i(\m{x}, \m{y}, \xi_{i})- \frac{N}{\ell_{g,1}}\nabla^2_{\m{xy}}g_i(\m{x},\m{y};{\zeta}_{i,N'+1}) \m{p}_{N'}) $%~~\Comment{via automatic differentiation}
% % \State  $\m{H}_i^{k+1} = \m{H}_i^k + \pi_1 \m{S}_i^k$ and $\m{J}_i^{k+1} = \m{J}_i^k + \pi_2\m{W}_i^k$;
% % %\State Send $\nabla f_i(x^k)$,\; $\mS_i^k \eqdef \cC_i^k(\nabla^2 f_i(x^k) - \mH_i^k)$ and $l_i^k \eqdef \|\mH_i^k - \nabla^2 f_i(x^k)\|_{\rm F}$ to the server
% %\State  $\m{x}^{+}=1/m\sum_{i\in\mathcal{S}}\m{x}_{i}$
% \EndFor
% \State  $\m{x}^{+}=1/|\mc{S}_{N'+1}|\sum_{i\in \mc{S}_{N'+1}} \m{x}_{i}$
% % \EndFor
% \end{algorithmic}
% \end{algorithm}
%  \end{subfigure}
%   \hspace*{0.03in}
%  \begin{subfigure}{.5\textwidth}
% \begin{algorithm}[H]
%   \caption*{$\m{x}^{+} ~=~\pmb{\fedout}~(\m{x}, \m{y}, \alpha,N$ }
% \begin{algorithmic}[1]
% %\For{$t=T-1,...,0$}
% \State Select $ N'\in \{1, \dots, N\}$ and $\mc{S}_0, \ldots, \mc{S}_{ N'+1} \in \mc{S}$ uniformly at random.
%   \For{$i \in \mc{S}_0$ \textbf{in parallel}} 
%  \State Compute $\nabla_y f_i(\m{x}, \m{y}; \xi_{i,n})$
%  \EndFor
%  \State $ \m{p}_0 \leftarrow 1/|\mc{S}_0|\sum_{i\in\mathcal{S}_0} \nabla_y f_i(\m{x}, \m{y}; \xi_{i,n})$ 
%  	%	\State $\m{p}_{i,0}\leftarrow \m{p}$
%  		 \For{$n=1,\ldots, N'$}
%  	   % \State Choose $N' \in \{0,\ldots,N-1\}$ randomly and 
% 	%	\For {$i \in \mc{S}$ \textbf{in parallel}} 
% 		\For {$i \in \mc{S}_n$ \textbf{in parallel}} 
% 		 \State $\m{p}_{i,n} \leftarrow (\m{I}-\frac{1}{\ell_{g,1}}\nabla^2_y g_i(\m{x}, \m{y};{\zeta}_{i,n}))\m{p}_{n-1}$% \Comment{$\m{X}_{i,j} := \nabla^2_y g_i(\m{x}, \m{y};\xi_j)$}
% 	   \EndFor
% 	   \State $\m{p}_{n}\leftarrow 1/|\mc{S}_n|\sum_{i\in|\mc{S}_n|} \m{p}_{i,n}$
% 	   %\Else 
%  	   %\State $\m{p}_{i}^{k,t}=\m{p}^{k,t+1}-\beta_i \nabla_\m{y}^2  g_i (\m{x},\m{y})\m{p}^{k,t+1}$~~ 
% 	   %\EndFor
% 	%	\State $\m{p}^{k,t}= 1/m\sum_{i\in\mathcal{S}} \m{p}_{i}^t$
% 	%	\State { $\m{p}^k=\sum_{t=0}^{T-1}\m{p}^{k,t}$}
% 		\EndFor
%  	%	\State $\m{p}_{N'}= 1/m\sum_{i\in\mathcal{S}} \m{p}_{i,N'}$ \som{Do we explicitly calculate this, or use HVP (ideal approach)? It should be clarified and we can discuss if needed.}
%  \For {$i \in \mc{S}_{N'+1}$ \textbf{in parallel}} 
%  \State $ \m{x}_{i}= \m{x}_i- \alpha (\nabla_{\m{x}} f_i(\m{x}, \m{y}, \xi_{i})- \frac{N}{\ell_{g,1}}\nabla^2_{\m{xy}}g_i(\m{x},\m{y};{\zeta}_{i,N'+1}) \m{p}_{N'}) $%~~\Comment{via automatic differentiation}
% % \State  $\m{H}_i^{k+1} = \m{H}_i^k + \pi_1 \m{S}_i^k$ and $\m{J}_i^{k+1} = \m{J}_i^k + \pi_2\m{W}_i^k$;
% % %\State Send $\nabla f_i(x^k)$,\; $\mS_i^k \eqdef \cC_i^k(\nabla^2 f_i(x^k) - \mH_i^k)$ and $l_i^k \eqdef \|\mH_i^k - \nabla^2 f_i(x^k)\|_{\rm F}$ to the server
% %\State  $\m{x}^{+}=1/m\sum_{i\in\mathcal{S}}\m{x}_{i}$
% \EndFor
% \State  $\m{x}^{+}=1/|\mc{S}_{N'+1}|\sum_{i\in \mc{S}_{N'+1}} \m{x}_{i}$
% % \EndFor
% \end{algorithmic}
% \end{algorithm}
%  \end{subfigure}
%   \vspace*{-0.15in}
% \end{figure*}

% \begin{algorithm}[t]
% \caption{~$\m{x}^{+} ~=~\pmb{\fedout}~(\m{x}, \m{y}, \alpha,N$ )
% %\colorbox{red!30}{\pmb{$\fedblo$}}, \colorbox{green!30}{\pmb{$\fedminmax$}}, and \colorbox{blue!20}{\pmb{$\fedcomp$}} 
% }
% \label{alg:fedinn}
% \begin{algorithmic}[1]
% %\For{$t=T-1,...,0$}
% \State Select $ N'\in \{1, \dots, N\}$ and $\mc{S}_0, \ldots, \mc{S}_{ N'+1} \in \mc{S}$ uniformly at random.
%   \For{$i \in \mc{S}_0$ \textbf{in parallel}} 
%  \State Compute $\nabla_y f_i(\m{x}, \m{y}; \xi_{i,n})$
%  \EndFor
%  \State $ \m{p}_0 \leftarrow 1/|\mc{S}_0|\sum_{i\in\mathcal{S}_0} \nabla_y f_i(\m{x}, \m{y}; \xi_{i,n})$ 
%  	%	\State $\m{p}_{i,0}\leftarrow \m{p}$
%  		 \For{$n=1,\ldots, N'$}
%  	   % \State Choose $N' \in \{0,\ldots,N-1\}$ randomly and 
% 	%	\For {$i \in \mc{S}$ \textbf{in parallel}} 
% 		\For {$i \in \mc{S}_n$ \textbf{in parallel}} 
% 		 \State $\m{p}_{i,n} \leftarrow (\m{I}-\frac{1}{\ell_{g,1}}\nabla^2_y g_i(\m{x}, \m{y};{\zeta}_{i,n}))\m{p}_{n-1}$% \Comment{$\m{X}_{i,j} := \nabla^2_y g_i(\m{x}, \m{y};\xi_j)$}
% 	   \EndFor
% 	   \State $\m{p}_{n}\leftarrow 1/|\mc{S}_n|\sum_{i\in|\mc{S}_n|} \m{p}_{i,n}$
% 	   %\Else 
%  	   %\State $\m{p}_{i}^{k,t}=\m{p}^{k,t+1}-\beta_i \nabla_\m{y}^2  g_i (\m{x},\m{y})\m{p}^{k,t+1}$~~ 
% 	   %\EndFor
% 	%	\State $\m{p}^{k,t}= 1/m\sum_{i\in\mathcal{S}} \m{p}_{i}^t$
% 	%	\State { $\m{p}^k=\sum_{t=0}^{T-1}\m{p}^{k,t}$}
% 		\EndFor
%  	%	\State $\m{p}_{N'}= 1/m\sum_{i\in\mathcal{S}} \m{p}_{i,N'}$ \som{Do we explicitly calculate this, or use HVP (ideal approach)? It should be clarified and we can discuss if needed.}
%  \For {$i \in \mc{S}_{N'+1}$ \textbf{in parallel}} 
%  \State $ \m{x}_{i}= \m{x}_i- \alpha (\nabla_{\m{x}} f_i(\m{x}, \m{y}, \xi_{i})- \frac{N}{\ell_{g,1}}\nabla^2_{\m{xy}}g_i(\m{x},\m{y};{\zeta}_{i,N'+1}) \m{p}_{N'}) $%~~\Comment{via automatic differentiation}
% % \State  $\m{H}_i^{k+1} = \m{H}_i^k + \pi_1 \m{S}_i^k$ and $\m{J}_i^{k+1} = \m{J}_i^k + \pi_2\m{W}_i^k$;
% % %\State Send $\nabla f_i(x^k)$,\; $\mS_i^k \eqdef \cC_i^k(\nabla^2 f_i(x^k) - \mH_i^k)$ and $l_i^k \eqdef \|\mH_i^k - \nabla^2 f_i(x^k)\|_{\rm F}$ to the server
% %\State  $\m{x}^{+}=1/m\sum_{i\in\mathcal{S}}\m{x}_{i}$
% \EndFor
% \State  $\m{x}^{+}=1/|\mc{S}_{N'+1}|\sum_{i\in \mc{S}_{N'+1}} \m{x}_{i}$
% % \EndFor
% \end{algorithmic}
% \label{alg:fedopt}
% \end{algorithm} 

==> FedNest_ _/sec/intro.tex <==
\vspace{-10pt}
\section{Introduction}
In the federated learning (FL) paradigm, multiple clients cooperate to learn a model under the orchestration of a central server \citep{mcmahan17fedavg} without directly exchanging local client data with the server or other clients. The locality of data distinguishes FL from traditional distributed optimization and also motivates new methodologies to address heterogeneous data across clients. Additionally, cross-device FL across many edge devices presents additional challenges since only a small fraction of clients participate in each round, and clients cannot maintain \emph{state} across rounds~\citep{kairouz2019advances}. 

Traditional distributed SGD methods are often unsuitable in FL and incur high communication costs. To overcome this issue, popular FL methods, such as \fedavg~\citep{mcmahan17fedavg}, use local client updates, i.e. clients update their models multiple times before communicating with the server (aka,~local SGD). Although \fedavg has seen great success, recent works have exposed convergence issues in certain settings~\citep{karimireddy2020scaffold,hsu2019measuring}. This is due to a variety of factors, including \emph{client drift}, where local models move away from globally optimal models due to objective and/or systems heterogeneity. 
%
\begin{figure*}[t]
\centering
\begin{tikzpicture}
    \node at (-3.2,-.4)[anchor=west] {\includegraphics[width=\linewidth/2]{figs/fednest-cartoon.pdf}};
    %\node at (-4.5,1)[anchor=west] %[scale=2,rotate=-20,opacity=0.7]{Placeholder Figure};
%\vspace{}
\node at (6,1.8)[anchor=west] [scale=1]{{Communication-efficiency:}};
    \node at (6.3,1.4)[anchor=west] {\checkbox \fedhess avoids explicit Hessian};
    \node at (6.3,1.0)[anchor=west] {\checkbox \lfedblo for local hypergradients};
    
    \node at (6,0.5)[anchor=west] [scale=1]{{Client heterogeneity:}};
    \node at (6.3,0.15)[anchor=west] {\checkbox \fedinn avoids client drift};
    
    \node at (6,-0.3)[anchor=west] [scale=1]{{Finite sample bilevel theory:}};
    \node at (6.3,-0.7)[anchor=west] {\checkbox Stochastic inner \& outer analysis};
    
    \node at (6,-1.1)[anchor=west] [scale=1]{{Specific nested optimization problems:}};
    \node at (6.3,-1.5)[anchor=west] {\checkbox {Bilevel}};
    \node at (6.3,-1.9)[anchor=west] {\checkbox {Minimax}};
    \node at (6.3,-2.3)[anchor=west] {\checkbox {Compositional}};
    %\node at (4,-1.1)[anchor=west] [scale=1]{Applications:};
    %\node at (4.3,-1.5)[anchor=west] {\checkbox Hyper-parameter optimization.};
    %\node at (4.3,-1.9)[anchor=west] {\checkbox Min-max problems};
\end{tikzpicture}
\vspace{-10pt}\caption{Depiction of federated bilevel nested optimization and high-level summary of \fedblo (Algorithm~\ref{alg:fednest}). At outer loop, \fedhess uses multiple rounds of matrix-vector products to facilitate hypergradient computation while only communicating vectors. At inner loop, \fedinn uses \textsc{FedSVRG} to avoid client drift and find the unique global minima. Both are crucial for establishing provable convergence of \fedblo.}
%bilevel convergence guarantees
\label{fig_main}
\vspace{-5pt}
\end{figure*}

Existing FL methods, such as \fedavg, are widely applied to stochastic problems with \emph{single-level} structure. Instead, many machine learning tasks -- such as adversarial learning \citep{madry2017towards}, meta learning~\citep{bertinetto2018meta}, hyperparameter optimization~\citep{franceschi2018bilevel}, reinforcement/imitation learning~\citep{wu2020finite,arora2020provable}, and neural architecture search~\citep{liu2018darts} -- admit \emph{nested} formulations that go beyond the standard single-level structure. Towards addressing such nested problems, bilevel optimization has received significant attention in the recent literature%to address such nested problems
~\citep{ghadimi2018approximation,hong2020two,ji2021bilevel}; albeit in non-FL settings. On the other hand, federated versions have been elusive perhaps due to the additional challenges surrounding heterogeneity, communication, and inverse Hessian approximation. 

\noindent\textbf{Contributions:} This paper addresses these challenges and develops~\textbf{\fedblo}: A federated machinery for nested problems with provable convergence and lightweight communication. \fedblo is composed of \textbf{\fedinn}: a federated stochastic variance reduction algorithm (\textsc{FedSVRG}) to solve the inner problem while avoiding client drift, and \textbf{\fedout}: a communication-efficient federated hypergradient algorithm for solving the outer problem. Importantly, we allow both inner \& outer objectives to be finite sums over heterogeneous client functions. \fedblo runs a variant of \textsc{FedSVRG} on inner \& outer variables in an alternating fashion as outlined in Algorithm~\ref{alg:fednest}. We make multiple algorithmic and theoretical contributions summarized below.%
%across clients 
\vspace{-.2cm}
\begin{myitemize}
%
\item \textbf{The variance reduction} of \fedinn enables robustness in the sense that local models converge to the globally optimal inner model {despite client drift/heterogeneity} unlike \fedavg. While \fedinn is similar to \textsc{FedSVRG}~\cite{konevcny2016federated} and \textsc{FedLin}~\cite{mitra2021linear}, we make two key contributions: (i) We leverage the global convergence of \fedinn to ensure accurate hypergradient computation which is crucial for our bilevel proof.  (ii) We establish new convergence guarantees for single-level stochastic non-convex \textsc{FedSVRG}, which are then integrated within our \fedout.
%
 \item \textbf{Communication efficient bilevel optimization}: Within \fedout, we develop an efficient federated method for hypergradient estimation that bypass Hessian computation. Our approach approximates the global Inverse Hessian-Gradient-Product (IHGP) via computation of matrix-vector products over few communication rounds.
 %
 \item \textbf{\lfedblo:} To further improve communication efficiency, we additionally propose a Light-\fedblo algorithm, which computes hypergradients locally and only needs a single communication round for the outer update. Experiments reveal that \lfedblo becomes very competitive as client functions become more homogeneous.
%
 \item \textbf{Unified federated nested theory:} We specialize our bilevel results to \emph{minimax} and \emph{compositional} optimization with emphasis on the former. For these, \fedblo significantly simplifies and leads to faster convergence. Importantly, our results are on par with the state-of-the-art non-federated guarantees for nested optimization literature without additional assumptions (Table~\ref{table:blo2:results}).% as %
 \item We provide extensive \textbf{numerical experiments} on bilevel and minimax optimization problems. These demonstrate the benefits of \fedblo, efficiency of \lfedblo, and shed light on tradeoffs surrounding communication, computation, and heterogeneity.  %Code is available at \url{https://github.com/ucr-optml/FedNest}.
 \end{myitemize}
 %spanning hyper-parameter \& hyper-representation optimization (



==> FedNest_ _/sec/numerics.tex <==
%
\vspace{-.2cm}
\section{Numerical Experiments}\label{sec:numerics}
In this section, we numerically investigate the impact of several attributes of our algorithms on a hyper-representation problem \cite{franceschi2018bilevel}, a hyper-parameter optimization problem for loss function tuning \cite{li2021autobalance}, and a federated minimax optimization problem. 

\subsection{Hyper-Representation Learning}
%In meta learning (ML), the representation is shared across all tasks. 
Modern approaches in meta learning such as MAML~\cite{finn2017model} and reptile \cite{nichol2018reptile} learn representations (that are shared across all tasks) in a bilevel manner. Similarly, the hyper-representation problem optimizes a classification model in a two-phased process. The outer objective optimizes the model backbone to obtain better feature representation on validation data. The inner problem optimizes a header for downstream classification tasks on training data. In this experiment, we use a 2-layer multilayer perceptron (MLP) with 200 hidden units. The outer problem optimizes the hidden layer with 157,000 parameters, and the inner problem optimizes the output layer with 2,010 parameters. We study both i.i.d and non-i.i.d. ways of partitioning the MNIST data exactly following~\textsc{FedAvg}~\cite{mcmahan17fedavg}, and split each client's data evenly to train and validation datasets. Thus, each client has 300 train and 300 validation samples. 

Figure~\ref{fig:hr_exp} demonstrates the impact on test accuracy of  several important components of \fednest. Figure~\ref{fig:hr_global_local} compares $\fednest$ and $\lfedblo$. Both algorithms perform well on the i.i.d. setup, while on the non-i.i.d. setup, $\fednest$ achieves i.i.d. performance, significantly outperforming $\lfedblo$. These findings are in line with our discussions in Section~\ref{light blo}. $\lfedblo$ saves on communication rounds compared to $\fednest$ and performs well on homogeneous clients. However, for heterogeneous clients, the isolation of local Hessian in $\lfedblo$ (see Algorithm~\ref{alg:localfedout} in Appendix~\ref{sec:simp:algs}) degrades the test performance.  Next, Figure~\ref{fig:hr_svrg_sgd} demonstrates the importance of SVRG in $\fedinn$ algorithm for heterogeneous data (as predicted by our theoretical considerations in Section~\ref{sec:fedinn}). To further clarify the algorithm difference in Figures~\ref{fig:hr_svrg_sgd} and \ref{fig:lt_global_local}, we use $\fednest_\mathrm{SGD}$ to denote the \fednest algorithm where SGD is used in \fedinn. Finally, Figure~\ref{fig:hr_tau} elucidates the role of local epoch $\tau$ in $\fedout$: larger $\tau$ saves on communication and improves test performance by enabling faster convergence.
%
\begin{figure}[t]
\vspace{-10pt}
    \centering
    \begin{subfigure}{0.226\textwidth}
    \centering
        \begin{tikzpicture}
        \node at (0,0) {\includegraphics[scale=0.256]{figs/global_local_epoch.pdf}};
        \node at (0,-1.65) [scale=0.7]{\textsc{FedNest} epochs};
        \node at (-2,0) [scale=0.7, rotate=90]{Balanced Test Accuracy};
        \end{tikzpicture}\vspace{-5pt}\caption{\textsc{FedNest} achieves similar performance as non-federated bilevel loss function tuning. }\label{fig:lt_global_local}
    \end{subfigure}\hspace{5pt}\begin{subfigure}{0.225\textwidth}
    \centering
        \begin{tikzpicture}
        \node at (0,0) {\includegraphics[scale=0.256]{figs/ib_optim_round.pdf}};
        \node at (0,-1.65) [scale=0.7]{Communication rounds};
        \end{tikzpicture}\vspace{-5pt}\caption{SVRG in $\fedinn$ provides better convergence and stability especially in non-iid setup.}\label{fig:lt_svrg_sgd}
    \end{subfigure}
    \vspace{-5pt}\caption{Loss function tuning on a 3-layer MLP and imbalanced MNIST dataset to maximize \emph{class-balanced test accuracy}. The \emph{brown dashed} line is the accuracy on non-federated bilevel optimization~\cite{li2021autobalance}, and the \emph{black dashed} line is the accuracy without tuning the loss function.}\label{fig:lt_exp}\vspace{-15pt}
\end{figure}

\subsection{Loss Function Tuning on Imbalanced Dataset}
We use bilevel optimization to tune a loss function for learning an imbalanced MNIST dataset. We aim to maximize the class-balanced validation accuracy (which helps minority/tail classes). Following the problem formulation in \cite{li2021autobalance}, we tune the so-called VS-loss function \cite{kini2021label} in a federated setting. In particular, we first create a long-tail imbalanced MNIST dataset by exponentially decreasing the number of examples per class (e.g.~class 0 has 6,000 samples, class 1 has 3,597 samples and finally, class 9 has only 60 samples). We partition the dataset to 100 clients following again $\fedavg$ \cite{mcmahan17fedavg} on both i.i.d.~and non-i.i.d.~setups. Different from the hyper-representation experiment, we employ 80\%-20\% train-validation on each client and use a 3-layer MLP model with 200, 100 hidden units, respectively. It is worth noting that, in this problem, the outer objective $f$ (aka validation cost) only depends on the hyperparameter $\m{x}$ through the optimal model parameters $\y^*(\x)$; thus, the direct gradient $\nabla^{\texttt{D}} f_i(\m{x},\m{y}^*(\m{x}))$ is zero for all $i \in\mc{S}$.

Figure~\ref{fig:lt_exp} displays test accuracy vs epochs/rounds for our federated bilevel algorithms. The horizontal dashed lines serve as non-FL baselines: brown depicts accuracy reached by bilevel optimization in non-FL setting, and, black depicts accuracy without any loss tuning. Compared to these, Figure~\ref{fig:lt_global_local} shows that $\fednest$ achieves near non-federated performance. In Figure~\ref{fig:lt_svrg_sgd}, we investigate the key role of SVRG in $\fedinn$ by comparing it with possible alternative implementation that uses SGD-type updates. The figure confirms our discussion in Section~\ref{sec:fedinn}: SVRG offers significant performance gains that are pronounced by client heterogeneity. %(e.g. compare blue to orange curve).

\subsection{Federated Minimax Problem}
\begin{figure}
\centering
\vspace{-5pt}
\begin{subfigure}{0.225\textwidth}
\centering
        \begin{tikzpicture}
        \node at (0,0) {\includegraphics[scale=0.255]{figs/minimax/mm_syn_y.pdf}};
        \node at (0,-1.45) [scale=0.7]{Epoch};
        \node at (-2,0) [scale=0.7, rotate=90]{$\|\y-\y^*\|^2$};
        \end{tikzpicture}\vspace{-5pt}
\end{subfigure}
\hspace{7pt}
\begin{subfigure}{0.225\textwidth}
    \centering
        \begin{tikzpicture}
        \node at (0,0) {\includegraphics[scale=0.255]{figs/minimax/mm_syn_x.pdf}};
        \node at (0,-1.45) [scale=0.7]{Epoch};
        \node at (-2,0) [scale=0.7, rotate=90]{$\|\x-\x^*\|^2$};
        \end{tikzpicture}\vspace{-5pt}
        %\caption{SVRG in $\fedinn$ provides better convergence and stability especially in non-iid setup.}\label{fig:lt_svrg_sgd}
\end{subfigure}\vspace{-5pt}
\caption{\textsc{FedNest} converges linearly despite heterogeneity. \textsc{LFedNest} slightly outperforms \textsc{FedAvg-S}.}\label{fig:mm}
\vspace{-10pt}
\end{figure}
%
We conduct experiments on the minimax problem \eqref{fedminmax:prob} with \[
f_i(\m{x},\m{y}):=-\left[\frac{1}{2}\|\m{y}\|^2 - \m{b}_i^\top \m{y} + \m{y}^\top \m{A}_i \m{x}\right] + \frac{\lambda}{2} \|\m{x}\|^2,
\]
to compare standard \textsc{FedAvg} saddle-point (\textsc{FedAvg}-S) method updating $(\m{x},\m{y})$ simultaneously~\cite{hou2021efficient} and our alternative approaches~(\textsc{LFedNest} and \textsc{FedNest}). This is a saddle-point formulation of $\min_{\m{x} \in \mb{R}^{d_1}} \frac{1}{2} \|\frac{1}{m} \sum_{i=1}^m \m{A}_i \m{x} - \m{b}_i\|^2$. %and is a typical example of minimax optimization used in literature. 
We set  $\lambda=10$, $\m{b}_i=\m{b}_i' - \frac{1}{m}\sum_{i=1}^m \m{b}_i'$ and $\m{A}_i = t_i \m{I}$, where $\m{b}_i' \sim \mathcal{N}(0, s^2 I_d)$, and $t_i$ is drawn UAR over $(0,0.1)$. Figure~\ref{fig:mm} shows that \textsc{LFedNest} and \textsc{FedNest} outperform \textsc{FedAvg}-S thanks to their alternating nature. \textsc{FedNest} significantly improves the convergence of \textsc{LFedNest} due to controlling client-drift. To our knowledge, \textsc{FedNest} is the only \textit{alternating} federated SVRG for minimax problems. 


==> FedNest_ _/sec/prelim.tex <==
\input{sec/table}
%
%\vspace{-10pt}
\section{Federated Nested Problems \& \fedblo}\label{sec:fedavg:full}
We will first provide the background on bilevel nested problems and then introduce our general federated method.

\noindent\textbf{Notation.}
$\mb{N}$ and $\mb{R}$ denotes the set of natural and real numbers, respectively. 
For a differentiable function $h(\m{x},\m{y}):\mb{R}^{d_1}\times\mb{R}^{d_2}\rightarrow\mb{R}$ in which $\m{y}=\m{y}(\m{x}):\mb{R}^{d_1}\rightarrow\mb{R}^{d_2}$, we denote $\nabla{h}\in\mb{R}^{d_1}$ the gradient of $h$ as a function of $\m{x}$ and  $\nabla_{\m{x}}{h}$, $\nabla_{\m{y}} h$ the partial derivatives of $h$ with respect to $\m{x}$ and $\m{y}$, respectively. We let $\nabla_{\m{xy}}^2 h$ and $\nabla_{\m{y}}^2 h$ denote the Jacobian and Hessian of $h$, respectively. We consider FL optimization over $m$ clients and we denote $\mathcal{S}=\{1,\ldots,m\}$. For vectors $\m{v} \in \mb{R}^d$ and matrix $\m{M} \in \mb{R}^{d \times d}$, we denote $\|\m{v}\|$ and $\|\m{M}\|$ the respective Euclidean and spectral norms.
%
\subsection{Preliminaries on Federated Nested Optimization}
In \textbf{federated bilevel learning}, we consider the  following nested optimization problem as depicted in Figure \ref{fig_main}:
%
\begin{subequations}\label{fedblo:prob}
\begin{align}
\begin{array}{ll}
\underset{\m{x} \in \mb{R}^{{d}_1}}{\min} &
\begin{array}{c}
f(\m{x})=\frac{1}{m} \sum_{i=1}^{m} f_{i}\left(\m{x},\m{y}^*(\m{x})\right) %{\rm\sf (outer)} 
\end{array}\\
\text{subj.~to} & \begin{array}[t]{l} \m{y}^*(\m{\m{x}})
%=
\in \underset{ \m{y}\in \mb{R}^{{d}_2}}{\textnormal{argmin}}~~\frac{1}{m}\sum_{i=1}^{m} g_i\left(\m{x},\m{y}\right). % ~~~~~~~~~~~~~~~~~~~~{\rm\sf (inner)} 
\end{array}
\end{array}
\end{align}
Recall that $m$ is the number of clients. Here, to model objective heterogeneity, each client $i$ is allowed to have its own individual outer \& inner functions $(f_i,g_i)$. Moreover, we consider a general stochastic oracle model, access to local functions $(f_i,g_i)$ is via stochastic sampling as follows:% over stochastic functions (e.g.~local client data)
\begin{align}
\nonumber 
 f_i(\m{x},\m{y}^*(\m{x})) &:= \mb{E}_{\xi \sim \mc{C}_i}\left[f_i(\m{x}, \m{y}^*(\m{x}); \xi)\right],\\g_i(\m{x},\m{y}) &:= \mb{E}_{\zeta \sim \mc{D}_i}\left[g_i(\m{x}, \m{y}; \zeta)\right],
\end{align}
\end{subequations}
%are the loss functions of the $i^{\text{th}}$ client, 
where $(\xi, \zeta)\sim(\mc{C}_i, \mc{D}_i)$ are  outer/inner sampling distributions for the $i^{\text{th}}$ client. We emphasize that for $i \neq j$, the tuples $(f_i,g_i,\mc{C}_i, \mc{D}_i)$ and $(f_j,g_j,\mc{C}_j, \mc{D}_j)$ can  be different.

\begin{example}[Hyperparameter tuning] Each client has local validation and training datasets associated with objectives $(f_i,g_i)_{i=1}^m$ corresponding to validation and training losses, respectively. The goal is finding hyper-parameters $\x$ that lead to learning model parameters $\y$ that minimize the (global) validation loss. 
\end{example}
%

\input{sec/fednest}
%\subsubsection{}
The stochastic bilevel problem \eqref{fedblo:prob} subsumes two popular problem classes with the nested structure: \emph{Stochastic MiniMax} \& \emph{Stochastic Compositional}. Therefore, results on the general nested problem \eqref{fedblo:prob}  also imply the results in these special cases. Below, we briefly describe them.



\textbf{Minimax optimization.} If $g_i(\x,\y;\zeta):=-f_i(\x,\y;\xi)$ for all $i \in \mc{S}$, the stochastic bilevel problem \eqref{fedblo:prob} reduces to the stochastic minimax problem
\begin{align}\label{fedminmax:prob}
\min_{\m{x}\in\mb{R}^{d_1}}~f(\m{x}):=\frac{1}{m} \max_{\m{y}\in\mb{R}^{d_2}}\sum_{i=1}^{m} \E[f_{i}\left(\m{x},\m{y}; \xi\right)].
\end{align}
%where $ f_i(\m{x},\m{y}^*(\m{x})) := \mb{E}_{\xi \sim \mc{C}_i}[f_i(\m{x}, \m{y}^*(\m{x}); \xi)]$. 
Motivated by applications in fair beamforming, training generative-adversarial networks (GANs) and robust machine learning, significant efforts have been made for solving \eqref{fedminmax:prob}~including \citep{daskalakis2018limit,gidel2018variational,mokhtari2020unified,thekumparampil2019efficient}.

\begin{example}[GANs] We train a generative model $g_{\x}(\cdot)$ and an adversarial model $a_{\y}(\cdot)$ using client datasets ${\mc{C}}_i$. The local functions may for example take the form $f_i(\x,\y)=\E_{s\sim {\mc{C}}_i}\{\log a_{\y}(s)\} +\E_{z\sim {\cal{D}}_{\text{noise}}}\{\log[1-a_{\y}(g_{\x}(z))]\}$.
\end{example}

\textbf{Compositional optimization.} Suppose $f_i(\m{x},\m{y};\xi):=f_i(\m{y};\xi)$ and $g_i$ is quadratic in $\m{y}$ given as $g_i(\m{x},\m{y};\zeta):=\|\m{y}-\m{r}_i(\m{x};\zeta)\|^2$. Then, the bilevel problem \eqref{fedblo:prob} reduces to 
%the compositional problem:
%\begin{subequations}
\begin{align}\label{fedcompos:prob2}
\begin{array}{ll}
\underset{\m{x} \in \mb{R}^{{d}_1}}{\min} &
\begin{array}{c}
f(\m{x})=\frac{1}{m} \sum_{i=1}^{m} f_{i}\left(\m{y}^*(\m{x})\right) %{\rm\sf (outer)} 
\end{array}\\
\text{subj.~to} & \begin{array}[t]{l} \m{y}^*(\m{\m{x}})=\underset{ \m{y}\in \mb{R}^{{d}_2}}{\textnormal{argmin}}~~\frac{1}{m}\sum_{i=1}^{m} g_i\left(\m{x},\m{y}\right) % ~~~~~~~~~~~~~~~~~~~~{\rm\sf (inner)} 
\end{array}
\end{array}
\end{align}
with $f_i(\m{y}^*(\m{x})) := \mb{E}_{\xi \sim \mc{C}_i}[f_i( \m{y}^*(\m{x}); \xi)]$ and $g_i(\m{x},\m{y}):= \mb{E}_{\zeta \sim \mc{D}_i}[g_i(\m{x},\m{y};\zeta)]$.
Optimization problems in the form of \eqref{fedcompos:prob2} occur for example in model agnostic meta-learning and policy evaluation in reinforcement learning \citep{finn2017model,ji2020theoretical,dai2017learning,wang2017stochastic}. 
%


\noindent \textbf{Assumptions.} Let $\m{z}=(\m{x},\m{y}) \in \mb{R}^{d_1+d_2}$. Throughout, we make the following assumptions on inner/outer objectives. 
\vspace{0.1cm}
% \noindent\textbf{Assumption 1 (Lipschitz continuity).}
%
\begin{assumption}[Well-behaved objectives]\label{assu:f} 
%\noindent   {\bf Assumptions A}
For all $i \in [m]$:
\begin{enumerate}[label={\textnormal{\textbf{(A\arabic*})}}]
%[label={\textbf{(a\arabic*})}]
\vspace{-.3cm}
\item %[\textbf{a)}]
$f_i(\m{z}), \nabla f_i(\m{z}), \nabla g_i(\m{z}), \nabla^2 g_i (\m{z})$ are $\ell_{f,0}$,$\ell_{f,1}$,$\ell_{g,1}$, $\ell_{g,2}$-Lipschitz continuous, respectively; and 
\vspace{-.2cm}
\item % [\textbf{d)}]
$g_i(\m{x},\m{y})$ is $\mu_{g}$-strongly convex in $\m{y}$ for all $\m{x}\in \mb{R}^{d_1}$.
\end{enumerate}
\end{assumption}
Throughout, we use $\kappa_g=\ell_{g,1}/\mu_g$ to denote the condition number of the inner function $g$.
\begin{assumption}[Stochastic samples]\label{assu:bound:var}
For all $i \in [m]$:
\begin{enumerate}[label={\textnormal{\textbf{(B\arabic*})}}]
\vspace{-.3cm}
\item $\nabla f_i(\m{z};\xi)$, $\nabla g_i(\m{z};\zeta)$, $\nabla^2 g_i(\m{z}; \zeta)$ are unbiased estimators of $\nabla f_i(\m{z})$, $\nabla g_i(\m{z})$, $\nabla^2g_i(\m{z})$, respectively; and
%$\mb{E}_{\xi}[\nabla f_i(\m{z};\xi)]=\nabla f_i(\m{z})$, $\mb{E}_{\zeta}[\nabla g_i(\m{z};\zeta)]=\nabla g_i(\m{z})$, $\mb{E}_{\zeta}[\nabla^2 g_i(\m{z}, \zeta)=\nabla g_i(\m{z})]$
%are unbiased estimators of $\nabla f_i(\m{z})$, $\nabla g_i(\m{z})$, and $\nabla^2g_i(\m{z})$, respectively;
\item Their variances are bounded, i.e., $\mb{E}_{\xi}[\|\nabla f_i(\m{z};\xi)-\nabla f_i(\m{z})\|^2] \leq \sigma_f^2$,   $\mb{E}_{\zeta}[\|\nabla g_i(\m{z};\zeta) -\nabla g_i(\m{z})\|^2] \leq \sigma_{g,1}^2$, and $\mb{E}_{\zeta}[\|\nabla^2 g_i(\m{z};\zeta)-\nabla^2 g_i(\m{z})\|^2] \leq \sigma_{g,2}^2$ for some $\sigma_f^2, \sigma_{g,1}^2$, and $\sigma_{g,2}^2$.
\end{enumerate}
\end{assumption}
These assumptions are common in the bilevel optimization literature~\citep{ghadimi2018approximation,chen2021closing,ji2021bilevel}. Assumption~\ref{assu:f} requires that the inner and outer functions are well-behaved. Specifically, strong-convexity of the inner objective is a recurring assumption in bilevel optimization theory implying a unique solution to the inner minimization in \eqref{fedblo:prob}.
%; see, e.g., \citep{ghadimi2018approximation,hong2020two,liu2021investigating}.
% Note that Assumptions~\ref{assu:f}--\ref{assu:bound:var} yield the following upper bound on the second moments, for all $i \in \{1,\ldots, m\}$:
% %\som{(2b) is not immediately clear to me due to spectral norm. However 2 times should be correct.}
% \begin{subequations}
% \begin{align}\label{eq.assp_grad_norm}
% &\mb{E}_{\xi}[\|\nabla f_i(\m{x},\m{y};\xi)\|^2]\leq \ell_{f,0}^2 + \sigma_f^2=:C_{f}^2,\\
% &\mb{E}_{\zeta}[\|\nabla^2 g_i(\m{x},\m{y};\zeta)\|^2]\leq \ell_{g,1}^2 + \sigma_{g,2}^2=:C_{g}^2.
% \end{align}
%\end{subequations}

==> FedNest_ _/sec/related.tex <==
%\vspace{-0.4cm}
\section{Related Work}
%To the best of our knowledge, \fednest is the first approach that can optimize a general bilevel optimization problem in a FL setting. Related work falls into two categories: federated learning and bilevel optimization. 
\noindent\textbf{Federated learning.} \fedavg  was first introduced by \citet{mcmahan17fedavg}, who showed it can dramatically reduce communication costs. For identical clients, \fedavg coincides with local SGD \cite{zinkevich2010parallelized} which has been analyzed by many works \citep{stich2018local,yu2019parallel,wang2018cooperative}. Recently, many variants of \fedavg  have been proposed to tackle issues such as convergence and client drift. Examples include \textsc{FedProx}~\cite{li2020federated}, \scaffold \cite{karimireddy2020scaffold},  \textsc{FedSplit} \cite{pathak2020fedsplit}, \textsc{FedNova}~\cite{wang2020tackling}, and, the most closely relevant to us \textsc{FedLin} \cite{mitra2021linear}. A few recent studies are also devoted to the extension of \fedavg to the minimax optimization~\cite{rasouli2020fedgan,deng2020distributionally} and compositional optimization~\cite{huang2021compositional}. In contrast to these methods, \fednest makes alternating SVRG updates between the global variables $\m{x}$ and $\m{y}$, and yields sample complexity bounds and batch size choices that are on par with the non-FL guarantees~(Table~\ref{table:blo2:results}). Evaluations in the Appendix \ref{sec:joinvsalt} reveal that both alternating updates and SVRG provides a performance boost over these prior approaches.

\noindent\textbf{Bilevel optimization.} This class of problems was first introduced by \cite{bracken1973mathematical}, and since then, different types of approaches have been proposed. See~\cite{sinha2017review,liu2021investigating} for surveys. 
 Earlier works in \cite{aiyoshi1984solution,lv2007penalty} reduced the bilevel problem to a single-level optimization problem. However, the reduced problem is still difficult to solve due to for example a large number of constraints. Recently, more efficient gradient-based  algorithms have been proposed by estimating the hypergradient of $\nabla f(\m{x})$ through iterative updates~\citep{maclaurin2015gradient,franceschi2017forward,domke2012generic,pedregosa2016hyperparameter}. The asymptotic and  non-asymptotic analysis of bilevel optimization has been provided in~\citep{franceschi2018bilevel,shaban2019truncated,liu2020generic} and \citep{ghadimi2018approximation,hong2020two}, respectively. There is also a line of work focusing on minimax optimization \cite{nemirovski2004prox,daskalakis2018limit} and compositional optimization~\cite{wang2017stochastic}. Closely related to our work are \cite{lin2020gradient,rafique2021weakly,chen2021closing} and \cite{ghadimi2020single,chen2021closing} which provide non-asymptotic analysis of SGD-type methods for minimax and compositional problems with outer nonconvex objective, respectively. 

A more in-depth discussion of related work is given in Appendix~\ref{supp:sec:related}. We summarize the complexities of different methods for FL/non-FL bilevel optimization in Table~\ref{table:blo2:results}.
%and \ref{table:blo2comps:results}.

==> FedNest_ _/sec/table.tex <==
\begin{table}[t]\vspace{-7pt}
\begin{minipage}[b]{1\linewidth}\centering
\scalebox{0.75}{\hspace*{-5pt}
\begin{tabular}{|l|c|c|c | c| }
\multicolumn{5}{c}{\large{Stochastic Bilevel Optimization}} \\
 \cline{3-5}
\multicolumn{2}{c}{}&\multicolumn{3}{|c|}{Non-Federated}\\
 \cline{2-5}
\multicolumn{1}{c|}{}&\textbf{\fednest} & \textbf{ALSET}  & \textbf{BSA} &  \textbf{TTSA}  \\
\hline
\textbf{batch size} &  \multicolumn{4}{c|}{${\cal O}(1)$}  \\
%\textbf{inner solver} &\fedinn& SGD  &\!\! SGD, ${\cal O}(\epsilon^{-1})$ \!\! & SGD   \\
%\textbf{outer solver} &\fedout & SGD \!\! & SGD &SGD   \\
\hline
 \makecell{\makecell{\textbf{samples in $\xi$}\\ \textbf{samples in $\zeta$}}}  & \makecell{ ${\cal O}(\kappa_g^5\epsilon^{-2})$ \\ ${\cal O}(\kappa_g^9 \epsilon^{-2})$ }& \makecell{ ${\cal O}( \kappa_g^5\epsilon^{-2})$ \\ ${\cal O}( \kappa_g^9\epsilon^{-2})$ } & \makecell{ ${\cal O}( \kappa_g^6\epsilon^{-2})$  \\ ${\cal O}(\kappa_g^9\epsilon^{-3})$ }  & \makecell{ ${\cal O}( \kappa_g^p\epsilon^{-2.5})$  \\ ${\cal O}( \kappa_g^p\epsilon^{-2.5})$ }
 \\ 
 \hline
%\hline
 \multicolumn{5}{c}{} \\
 \multicolumn{5}{c}{\large{Stochastic Minimax Optimization}} \\
%\hline
 \cline{3-5}
\multicolumn{2}{c|}{}&\multicolumn{3}{c|}{Non-Federated}\\
 \cline{2-5}
\multicolumn{1}{c|}{}&\textbf{\fednest}	& \textbf{ALSET}  & \textbf{SGDA} &  \textbf{SMD}      \\ 
\hline
\textbf{batch size} & \mc{O}(1) & ${\cal O}(1)$   & ${\cal O}(\epsilon^{-1})$  & N.A.  \\ 
%\textbf{\textbf{inner solver}} &\fedinn & SGD  & SGD& subproblem         \\ 
%\textbf{\textbf{outer solver}} &\fedout & SGD  & SGD& SGD         \\ 
\hline
\textbf{samples }  & \multicolumn{4}{c|}{${\cal O}(\kappa^3_f\epsilon^{-2})$}
%& ${\cal O}(\kappa^3_f\epsilon^{-2})$  &  ${\cal O}(\kappa^3_f\epsilon^{-2})$
\\ 
 \hline
 \multicolumn{5}{c}{} \\
\multicolumn{5}{c}{\large{Stochastic Compositional Optimization}} \\
%\hline
 \cline{3-5}
\multicolumn{2}{c}{}&\multicolumn{3}{|c|}{Non-Federated}\\
 \cline{2-5}
\multicolumn{1}{c|}{}&\textbf{\fednest}	& \textbf{ALSET}  & \textbf{SCGD} & \textbf{NASA}      
\\ \hline
\textbf{batch size} & \multicolumn{4}{c|}{${\cal O}(1)$} 
%\\ \hline
%\textbf{$y$-update} &\fedinn &SGD  & SGD& correction     
\\ \hline
\textbf{samples}  &$ {\cal O}(\epsilon^{-2})$& ${\cal O}(\epsilon^{-2})$  & ${\cal O}(\epsilon^{-4})$  & ${\cal O}(\epsilon^{-2})$ \\ 
\hline
%\hline
 \end{tabular}
}
\vspace{-0.1cm}
\caption{\small{Sample complexity of \fedblo and comparable non-FL methods to find an $\epsilon$-stationary point of $f$: $\kappa_g:=\ell_{g,1}/\mu_g$ and $\kappa_f:=\ell_{f,1}/\mu_f$.  $\kappa^p_g$ denotes a polynomial function of $\kappa_g$.  {ALSET} \citep{chen2021closing}, {BSA} \citep{ghadimi2018approximation}, {TTSA} \citep{hong2020two}, SGDA \citep{lin2020gradient}, SMD \citep{rafique2021weakly}, SCGD~\citep{wang2017stochastic}, and NASA~\citep{ghadimi2020single}. 
}}
\label{table:blo2:results}
\vspace{-0.35cm}
\end{minipage}%\vspace{-0.5cm}
\end{table}%\vspace{-0.15cm}


==> FedNest_ _/sec/theory.tex <==
\section{Convergence Analysis for \fedblo}\label{sec:theory}
In this section, we present convergence results for \fedblo. All proofs are relegated to Appendices~\ref{sec:app:bilevel}--\ref{sec:app:compos}.% due to space constraints.
\begin{theorem}\label{thm:fednest}
Suppose Assumptions~\ref{assu:f} and \ref{assu:bound:var} hold.  Further, assume  $\alpha_i^k=\alpha_k/\tau_i$ and $\beta_i^k=\beta_k/\tau_i$ for all $ i \in \mathcal{S}$, where 
%\begin{subequations}\label{eqn:parrr}
\begin{align}\label{eqn:param:choice}
%&\tau_i\geq 1,\forall i\in\mc{S},~~~\beta_i=\frac{{\beta}_k}{\tau_i},~~\textnormal{where}~~
\beta_k &= \frac{\bar{\beta} \alpha_k}{T},~~~\alpha_k=\min\left\{\bar{\alpha}_1, \bar{\alpha}_2, \bar{\alpha}_3, \frac{\bar{\alpha}}{\sqrt{K}}\right\}
\end{align}
%\end{subequations}
for some positive constants $\bar\alpha_1,\bar\alpha_2,\bar\alpha_3,\bar{\alpha}$, and $\bar{\beta}$ independent of $K$. Then, for any $T\geq 1$, the iterates $\{(\m{x}^k,\m{y}^k)\}_{k\geq0}$ generated by \fednest satisfy
%\begin{subequations}
\begin{equation*}
\begin{aligned}%\label{eq.theorem1}
 \frac{1}{K} \sum_{k=1}^K\mb{E}\left[\left\|\nabla f(\m{x}^k)\right\|^2\right] =~&{\cal O}\Big(\frac{\bar{\alpha}\max(\sigma_{g,1}^2, \sigma_{g,2}^2,\sigma_f^2)}{\sqrt{K}} \\
& + \frac{1}{\min(\bar{\alpha}_1, \bar{\alpha}_2, \bar{\alpha}_3)K} + b^2 \Big),
\end{aligned}
\end{equation*}
%\end{subequations}
where  $b=\kappa_g\ell_{f,1}\big( (\kappa_g-1)/\kappa_g \big)^{N}$ and $N$ is the input parameter to \fedhess.
%b:= \frac{\ell_{g,1} \ell_{f,1}}{\mu_g} \big( \frac{\kappa_g-1}{\kappa_g} \big)^{N}
%where $\m{y}^\star(\m{x}^K)$ is the minimizer of the inner problem in \eqref{fedblo:prob}.
\end{theorem}
%
%
%\begin{subequations}
\begin{corollary}[\textbf{Bilevel}]\label{thm:fednest:bilevel}
Under the same conditions as in Theorem \ref{thm:fednest},  if
{\small $N={\cal O}(\kappa_g \log K)$ and $T=\mc{O}(\kappa_g^{4})$}, then 
\begin{equation*}
 \frac{1}{K} \sum_{k=1}^K\mb{E}\left[\left\|\nabla f(\m{x}^k)\right\|^2\right]= \mc{O}\left(\frac{\kappa_g^4}{K} + \frac{\kappa_g^{2.5}}{\sqrt{K}}\right).
\end{equation*}
For $\epsilon$-accurate stationary point, we need $K=\mc{O}(\kappa^5_g \epsilon^{-2})$.
\end{corollary}
Above, we choose $N\propto \kappa_g \log K$ to guarantee $b^2\lesssim 1/\sqrt{K}$. In contrast, we use $T\gtrsim\kappa_g^4$ inner SVRG epochs. From Section~\ref{light blo}, this would imply the communication cost is dominated by SVRG epochs $N$ and $\order{\kappa_g^4}$ rounds. 

From Corollary~\ref{thm:fednest:bilevel}, we remark that \fednest matches the guarantees of non-federated alternating SGD methods, such as ALSET~\cite{chen2021closing} and  {BSA} \citep{ghadimi2018approximation}, despite federated setting, i.e. communication challenge, heterogeneity in the client objectives, and device heterogeneity.
%
\begin{figure*}
\vspace{-10pt}
    \centering
    \begin{subfigure}{0.31\textwidth}
    \centering
        \begin{tikzpicture}
        \node at (0,0) {\includegraphics[scale=0.33]{figs/hr_global_local_epoch.pdf}};
        \node at (0,-2.1) [scale=0.9]{\textsc{FedNest} epochs};
        \node at (-2.6,0) [scale=0.9, rotate=90]{Test accuracy};
        \end{tikzpicture}\vspace{-5pt}\caption{Comparison between \textsc{FedNest} and \textsc{LFedNest}.}
        \label{fig:hr_global_local}
    \end{subfigure}\hspace{5pt}\begin{subfigure}{0.31\textwidth}
    \centering
        \begin{tikzpicture}
        \node at (0,0) {\includegraphics[scale=0.33]{figs/hr_optim_round.pdf}};
        \node at (0,-2.1) [scale=0.9]{Communication rounds};
        
        \end{tikzpicture}\vspace{-5pt}\caption{SVRG in \fedinn provides better convergence and stability.}\label{fig:hr_svrg_sgd}
    \end{subfigure}\hspace{5pt}\begin{subfigure}{0.31\textwidth}
    \centering
        \begin{tikzpicture}
        \node at (0,0) {\includegraphics[scale=0.33]{figs/hr_tau_round.pdf}};
        \node at (0,-2.1) [scale=0.9]{Communication rounds};
        \end{tikzpicture}\vspace{-5pt}\caption{Larger $\tau$ in \fedout provides better performance.}\label{fig:hr_tau}
    \end{subfigure}\vspace{-6pt}\caption{Hyper-representation experiments on a 2-layer MLP and MNIST dataset.}\label{fig:hr_exp}
    \vspace{-8pt}
\end{figure*}
\vspace{-.3cm}
%
\subsection{Minimax Federated Learning}
We focus on special features of federated minimax problems and customize the general results to yield improved convergence results for this special case. Recall from \eqref{fedminmax:prob} that $g_i(\x,\y)=-f_i(\x,\y)$ which implies that $b=0$ and following Assumption \ref{assu:f},  $f_i(\x,\y)$ is $\mu_f$--strongly concave in $\y$ for all $\x$.
%
\begin{corollary}[\textbf{Minimax}]\label{thm:fednest:minmax}
Denote $\kappa_f=\ell_{f,1}/\mu_f$. Assume same conditions as in Theorem~\ref{thm:fednest}  and 
%except that $f (\cdot, \m{y})$ is only Lipchitz over $\m{x}$ but note that $f (\m{x}, \cdot)$ is Lipchitz continuous over $\m{y}$. 
 $T=\mc{O}(\kappa_f)$. Then, 
\begin{equation*}
 \frac{1}{K} \sum_{k=1}^K\mb{E}\left[\left\|\nabla f(\m{x}^k)\right\|^2\right]=\mc{O}\left(\frac{\kappa^2_f}{K} + \frac{\kappa_f}{\sqrt{K}}\right).
\end{equation*}
\end{corollary}
%
Corrollary~\ref{thm:fednest:minmax} implies that for the minimax problem, the convergence rate of \fedblo to the stationary point of $f$ is  $\mc{O}({1/\sqrt{K}})$. Again, we note this matches the convergence rate of non-FL algorithms (see also Table~\ref{table:blo2:results}) such as SGDA \citep{lin2020gradient} and SMD~\citep{rafique2021weakly}.
%
\subsection{Compositional Federated Learning}
Observe that in the compositional problem~\eqref{fedcompos:prob2}, the outer function is $f_i(\m{x},\m{y};\xi)=f_i(\m{y};\xi)$ and the inner function is  $g_i(\m{x},\m{y};\zeta)=\frac{1}{2}\|\m{y}-\m{r}_i(\m{x};\zeta)\|^2$, for all $i \in \mc{S}$. Hence, $b=0$ and $\kappa_g=1$. %
\begin{corollary}[\textbf{Compositional}]\label{thm:fednest:compos}
Under the same conditions as in Theorem \ref{thm:fednest}, if we select $T=1$ in \eqref{eqn:param:choice}. Then,
\begin{equation*}
 \frac{1}{K} \sum_{k=1}^K\mb{E}\left[\left\|\nabla f(\m{x}^k)\right\|^2\right]=\mc{O}\left(\frac{1}{\sqrt{K}}\right).
\end{equation*}
\end{corollary}
%
Corrollary~\ref{thm:fednest:compos} implies that for the  compositional problem \eqref{fedcompos:prob2}, the convergence rate of \fedblo to the stationary point of $f$ is  $\mc{O}({1/\sqrt{K}})$. This matches the convergence rate of non-federated stochastic algorithms such as SCGD~\citep{wang2017stochastic} and NASA~\citep{ghadimi2020single} (Table~\ref{table:blo2:results}).
%
%
\subsection{Single-Level Federated Learning}
Building upon the general results for stochastic nonconvex nested problems, we establish new convergence guarantees for \emph{single-level} stochastic non-convex federated SVRG which is integrated within our \fedout.  Note that in the single-level setting,  the optimization problem~\eqref{fedblo:prob} reduces to 
\begin{align}\label{fedsingle:prob2}
\underset{\m{x} \in \mb{R}^{{d}_1}}{\min} ~~f(\m{x})=\frac{1}{m} \sum_{i=1}^{m} f_{i}\left(\m{x}\right)
\end{align}
with $f_i(\m{x}) := \mb{E}_{\xi \sim \mc{C}_i}[f_i(\m{x}; \xi)]$, where  $\xi\sim\mc{C}_i$ is sampling distribution for the $i^{\text{th}}$ client.


We make the following assumptions on \eqref{fedsingle:prob2} that are counterparts of Assumptions~\ref{assu:f} and \ref{assu:bound:var}.
\begin{assumption}[Lipschitz continuity]\label{assu:s:f} 
For all $i \in [m]$, $\nabla f_i(\m{x})$ is $L_f$-Lipschitz continuous.
\end{assumption}
%Throughout, we use $\kappa_g=\ell_{g,1}/\mu_g$ to denote the condition number of the inner function $g$.
\begin{assumption}[Stochastic samples]\label{assu:s:bound:var}
For all $i \in [m]$, $\nabla f_i(\m{x};\xi)$ is an unbiased estimator of $\nabla f_i(\m{x})$ and its variance is bounded, i.e., $\mb{E}_{\xi}[\|\nabla f_i(\m{x};\xi)-\nabla f_i(\m{x})\|^2] \leq \sigma_f^2$.
\end{assumption}
%
\begin{theorem}[\textbf{Single-Level}]\label{thm:fednest:s:level}
Suppose Assumptions~\ref{assu:s:f} and \ref{assu:s:bound:var} hold.  Further, assume  $\alpha_i^k=\alpha_k/\tau_i$ for all $ i \in \mathcal{S}$, where 
\begin{align}\label{eqn:param:s:choice}
\alpha_k&=\min\left\{\bar{\alpha}_1,\frac{\bar{\alpha}}{\sqrt{K}}\right\}
\end{align}
for some positive $\bar{\alpha}_1$ and  $\bar{\alpha}$. Then,
\begin{equation*}
 \frac{1}{K} \sum_{k=1}^K\mb{E}\left[\left\|\nabla f(\m{x}^k)\right\|^2\right]=\mc{O}\left( \frac{ \Delta_f}{ \bar{\alpha}_1 K} + \frac{  \frac{\Delta_f}{\bar{\alpha}} + \bar{\alpha}\sigma_f^2 }{\sqrt{K}}\right),
\end{equation*}
where $\Delta_{f}:= f(\m{x}^0)-\mb{E}[f(\m{x}^K)]$.
\end{theorem}
Theorem~\ref{thm:fednest:s:level} extends recent results by \cite{mitra2021linear} from the stochastic strongly convex to the stochastic nonconvex setting. The above rate is also consistent with existing single-level non-FL guarantees~\cite{ghadimi2013stochastic}.

==> notation.tex <==
\usepackage[margin=1in]{geometry}
\renewcommand{\baselinestretch}{1.5}	% Line Stretch
\usepackage{color}
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{natbib}
\usepackage{caption}
\usepackage{longtable}
\usepackage{boldline}
% \usepackage[toc,page,header]{appendix}
% \usepackage{minitoc}
% Make the "Part I" text invisible
\renewcommand \thepart{}
\renewcommand \partname{}
\usepackage[colorlinks,citecolor=blue,linkcolor=blue,urlcolor=blue]{hyperref}
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{booktabs}
\usepackage[table,x11names,dvipsnames,table]{xcolor}
\usepackage{graphicx}
\usepackage{wrapfig}
\usepackage[rightcaption]{sidecap}
\sidecaptionvpos{figure}{c}
\usepackage{bbm}
\usepackage{latexsym, epsfig, amssymb, amsmath, amsthm, graphicx, mathrsfs, booktabs,mathtools}
\usepackage{enumerate}
\usepackage{multirow}
\usepackage{multicol}
\usepackage{array,booktabs}
\usepackage{enumitem}
\usepackage{epstopdf}
\usepackage{subcaption}
\usepackage{wrapfig}
\usepackage{adjustbox}
\usepackage{multirow}
\usepackage{multicol}
\usepackage{array,booktabs}
\usepackage{algorithm}
\usepackage{algpseudocode} 
\usepackage{enumitem}
\usepackage{epstopdf}
\usepackage{xspace}
\usepackage{comment}
\usepackage{multirow}
\usepackage{makecell}
\newcommand{\vct}[1]{\bm{#1}}
\newcommand{\mtx}[1]{\bm{#1}}
\newcommand{\x}{\vct{x}}
\newcommand{\y}{\vct{y}}


%%%
%%
%\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\renewcommand{\algorithmicrequire}{ \textbf{Input:}}
\renewcommand{\algorithmicensure}{ \textbf{Output:}}
\newcommand\inner[2]{\langle #1, #2 \rangle}
%%%%%
%%%% notation %%%%%%%%%%%%%%%%
\newcommand{\mc}{\mathcal}
\newcommand{\m}[1]{{\bf{#1}}}
\newcommand{\wh}[1]{{\widehat{#1}}}
\newcommand{\un}[1]{{\underline{#1}}}
\newcommand{\ti}[1]{{\tilde{#1}}}
\renewcommand{\mc}[1]{\ensuremath{\mathcal{#1}}} 
\newcommand{\g}[1]{\mbox{\boldmath $#1$}}
\newcommand{\mb}[1]{{\mathbb{#1}}}
\newcommand{\V}[1]{\ensuremath{\boldsymbol{#1}}\xspace}
\newcommand{\M}[1]{\ensuremath{\boldsymbol{#1}}\xspace}
%% Math Functions
\newcommand{\F}[1]{\ensuremath{\mathrm{#1}}\xspace}
\newcommand{\sgn}{\F{sgn}}
\newcommand{\tr}{\F{trace}}
%\newcommand{\text{diag}}{\F{diag}}
\newcommand{\dett}{\F{det}}
%\DeclareMathOperator*{\argmax}{\arg\!\max}
%\DeclareMathOperator*{\argmin}{\arg\!\min}
\DeclarePairedDelimiterX{\norm}[1]{\lVert}{\rVert}{#1}
\newcommand*{\Scale}[2][4]{\scalebox{#1}{$#2$}}
%% Transpose
%%%%% operator%%%%%%%%%%%% 
\DeclareMathOperator*{\minimize}{minimize}
%\DeclareMathOperator{\text{diag}}{diag}
\DeclareMathOperator{\trace}{trace}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\eig}{eig}
\DeclareMathOperator{\logt}{logdet}
\DeclareMathOperator{\Var}{Var}
%%%%%%%%%%% theorem %%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\Lmax}{\ensuremath{L^\ast}}
\newcommand{\Lsum}{\overline{L}}
\newcommand{\ellmin}{\ensuremath{\ell_\ast}}
\newcommand{\proxjplain}{ {\mathtt{prox\_update}}_j}
\newcommand{\proxj}[1]{\ensuremath{\proxjplain(#1)}}
\newcommand{\zfp}{z^\star}
\DeclareMathOperator{\refl}{\bf refl}
\newcommand{\aprox}{\widetilde{\prox}}
\newcommand{\aproxj}[2]{\mathtt{prox\_update}_{#1}(#2)}
\newcommand{\arefl}{\widetilde{\refl}}
\newcommand{\eqset}{E}
\newcommand{\Orthog}{\ensuremath{\mathrm{O}}}
\newcommand{\zstar}{z^\star}
\definecolor{darkred}{RGB}{150,0,0}
\definecolor{darkgreen}{RGB}{0,150,0}
\definecolor{darkblue}{RGB}{0,0,200}
\hypersetup{colorlinks=true, linkcolor=darkred, citecolor=darkgreen, urlcolor=darkblue}
\newcommand{\som}[1]{\marginpar{\color{darkred}\tiny\ttfamily SO: #1}}
\newcommand{\so}[1]{\textcolor{darkred}{#1}}
\newcommand{\SO}[1]{\textcolor{darkred}{SO: #1}}
\let\phi\varphi
\newcommand{\Unif}{\ensuremath{\mathsf{Unif}}}
\newcommand{\numepoch}{\numepochs}
\newcommand{\defn}{\ensuremath{\coloneq}}
%%%%
\newtheorem{theorem}{Theorem}[section] %[section]
\newtheorem{lemma}{Lemma}[section] %[section]
\newtheorem{corollary}{Corollary}[section] %[section]
\newtheorem{proposition}{Proposition}[section] %[section]
\newtheorem{definition}{Definition}[section] %[section]
\newtheorem{remark}{Remark}[section]%[section]
\newtheorem{example}{Example}[section] %[section]
\newtheorem{assumption}{Assumption}
\renewcommand*{\theassumption}{\Alph{assumption}}
%--------------------------------------------------------------
\newenvironment{myitemize}{\begin{list}{$\bullet$}
		{\setlength{\topsep}{1mm}
			\setlength{\itemsep}{0.25mm}
			\setlength{\parsep}{0.25mm}
			\setlength{\itemindent}{0mm}
			\setlength{\partopsep}{0mm}
			\setlength{\labelwidth}{15mm}
			\setlength{\leftmargin}{4mm}}}{\end{list}}

% Full names of federated algorithms
\newcommand{\fedblo}{\textsc{FedNest}\xspace}
\newcommand{\Blo}{Bilevel}
\newcommand{\blo}{bilevel}
\newcommand{\nn}{\nonumber}
\newcommand{\fed}{\textsc{Fed}\xspace}
\newcommand{\fadagrad}{\textsc{FedAdagrad}\xspace}
\newcommand{\fedavg}{\textsc{FedAvg}\xspace}
\newcommand{\fedavgm}{\textsc{FedAvgM}\xspace}
\newcommand{\fedopt}{\textsc{FedOpt}\xspace}
\newcommand{\fedesj}{\textsc{FedEsj}\xspace}
\newcommand{\fedsvrg}{\textsc{FedSVRG}\xspace}
\newcommand{\scaffold}{\textsc{SCAFFOLD}\xspace}
\newcommand{\adaalter}{\textsc{AdaAlter}\xspace}
\newcommand{\lookahead}{\textsc{Lookahead}\xspace}
\newcommand{\fedgrad}{\textsc{ApproxInverseHVP}\xspace}
\newcommand{\fedminmax}{\textsc{FedMinMax}\xspace}
\newcommand{\fedcomp}{\textsc{FedComp}\xspace}
\newcommand{\fedinn}{\textsc{FedInn}\xspace}
\newcommand{\fedout}{\textsc{FedOut}\xspace}
\newcommand{\fednest}{\textsc{FedNest}\xspace}
\newcommand{\fedhess}{\textsc{FedIHGP}\xspace}
